Code2Que: A Tool for Improving Question Titles from Mined Code Snippets in Stack Overflow

Stack Overflow is one of the most popular technical Q&A sites used by software developers. Seeking help from Stack Overflow has become an essential part of software developers' daily work for solving programming-related questions. Although the Stack Overflow community has provided quality assurance guidelines to help users write better questions, we observed that a significant number of questions submitted to Stack Overflow are of low quality. In this paper, we introduce a new web-based tool, Code2Que, which can help developers in writing higher quality questions for a given code snippet. Code2Que consists of two main stages: offline learning and online recommendation. In the offline learning phase, we first collect a set of good quality <code snippet, question> pairs as training samples. We then train our model on these training samples via a deep sequence-to-sequence approach, enhanced with an attention mechanism, a copy mechanism and a coverage mechanism. In the online recommendation phase, for a given code snippet, we use the offline trained model to generate question titles to assist less experienced developers in writing questions more effectively. At the same time, we embed the given code snippet into a vector and retrieve the related questions with similar problematic code snippets.

==> fontawesomesymbols-generic.tex <==
\def\faGlass{\faicon{glass}}
\def\faMusic{\faicon{music}}
\def\faSearch{\faicon{search}}
\def\faEnvelopeO{\faicon{envelope-o}}
\def\faHeart{\faicon{heart}}
\def\faStar{\faicon{star}}
\def\faStarO{\faicon{star-o}}
\def\faUser{\faicon{user}}
\def\faFilm{\faicon{film}}
\def\faThLarge{\faicon{th-large}}
\def\faTh{\faicon{th}}
\def\faThList{\faicon{th-list}}
\def\faCheck{\faicon{check}}
\def\faTimes{\faicon{times}}
\def\faSearchPlus{\faicon{search-plus}}
\def\faSearchMinus{\faicon{search-minus}}
\def\faPowerOff{\faicon{power-off}}
\def\faSignal{\faicon{signal}}
\def\faCog{\faicon{cog}}
\def\faTrashO{\faicon{trash-o}}
\def\faHome{\faicon{home}}
\def\faFileO{\faicon{file-o}}
\def\faClockO{\faicon{clock-o}}
\def\faRoad{\faicon{road}}
\def\faDownload{\faicon{download}}
\def\faArrowCircleODown{\faicon{arrow-circle-o-down}}
\def\faArrowCircleOUp{\faicon{arrow-circle-o-up}}
\def\faInbox{\faicon{inbox}}
\def\faPlayCircleO{\faicon{play-circle-o}}
\def\faRepeat{\faicon{repeat}}
\def\faRefresh{\faicon{refresh}}
\def\faListAlt{\faicon{list-alt}}
\def\faLock{\faicon{lock}}
\def\faFlag{\faicon{flag}}
\def\faHeadphones{\faicon{headphones}}
\def\faVolumeOff{\faicon{volume-off}}
\def\faVolumeDown{\faicon{volume-down}}
\def\faVolumeUp{\faicon{volume-up}}
\def\faQrcode{\faicon{qrcode}}
\def\faBarcode{\faicon{barcode}}
\def\faTag{\faicon{tag}}
\def\faTags{\faicon{tags}}
\def\faBook{\faicon{book}}
\def\faBookmark{\faicon{bookmark}}
\def\faPrint{\faicon{print}}
\def\faCamera{\faicon{camera}}
\def\faFont{\faicon{font}}
\def\faBold{\faicon{bold}}
\def\faItalic{\faicon{italic}}
\def\faTextHeight{\faicon{text-height}}
\def\faTextWidth{\faicon{text-width}}
\def\faAlignLeft{\faicon{align-left}}
\def\faAlignCenter{\faicon{align-center}}
\def\faAlignRight{\faicon{align-right}}
\def\faAlignJustify{\faicon{align-justify}}
\def\faList{\faicon{list}}
\def\faOutdent{\faicon{outdent}}
\def\faIndent{\faicon{indent}}
\def\faVideoCamera{\faicon{video-camera}}
\def\faPictureO{\faicon{picture-o}}
\def\faPencil{\faicon{pencil}}
\def\faMapMarker{\faicon{map-marker}}
\def\faAdjust{\faicon{adjust}}
\def\faTint{\faicon{tint}}
\def\faPencilSquareO{\faicon{pencil-square-o}}
\def\faShareSquareO{\faicon{share-square-o}}
\def\faCheckSquareO{\faicon{check-square-o}}
\def\faArrows{\faicon{arrows}}
\def\faStepBackward{\faicon{step-backward}}
\def\faFastBackward{\faicon{fast-backward}}
\def\faBackward{\faicon{backward}}
\def\faPlay{\faicon{play}}
\def\faPause{\faicon{pause}}
\def\faStop{\faicon{stop}}
\def\faForward{\faicon{forward}}
\def\faFastForward{\faicon{fast-forward}}
\def\faStepForward{\faicon{step-forward}}
\def\faEject{\faicon{eject}}
\def\faChevronLeft{\faicon{chevron-left}}
\def\faChevronRight{\faicon{chevron-right}}
\def\faPlusCircle{\faicon{plus-circle}}
\def\faMinusCircle{\faicon{minus-circle}}
\def\faTimesCircle{\faicon{times-circle}}
\def\faCheckCircle{\faicon{check-circle}}
\def\faQuestionCircle{\faicon{question-circle}}
\def\faInfoCircle{\faicon{info-circle}}
\def\faCrosshairs{\faicon{crosshairs}}
\def\faTimesCircleO{\faicon{times-circle-o}}
\def\faCheckCircleO{\faicon{check-circle-o}}
\def\faBan{\faicon{ban}}
\def\faArrowLeft{\faicon{arrow-left}}
\def\faArrowRight{\faicon{arrow-right}}
\def\faArrowUp{\faicon{arrow-up}}
\def\faArrowDown{\faicon{arrow-down}}
\def\faShare{\faicon{share}}
\def\faExpand{\faicon{expand}}
\def\faCompress{\faicon{compress}}
\def\faPlus{\faicon{plus}}
\def\faMinus{\faicon{minus}}
\def\faAsterisk{\faicon{asterisk}}
\def\faExclamationCircle{\faicon{exclamation-circle}}
\def\faGift{\faicon{gift}}
\def\faLeaf{\faicon{leaf}}
\def\faFire{\faicon{fire}}
\def\faEye{\faicon{eye}}
\def\faEyeSlash{\faicon{eye-slash}}
\def\faExclamationTriangle{\faicon{exclamation-triangle}}
\def\faPlane{\faicon{plane}}
\def\faCalendar{\faicon{calendar}}
\def\faRandom{\faicon{random}}
\def\faComment{\faicon{comment}}
\def\faMagnet{\faicon{magnet}}
\def\faChevronUp{\faicon{chevron-up}}
\def\faChevronDown{\faicon{chevron-down}}
\def\faRetweet{\faicon{retweet}}
\def\faShoppingCart{\faicon{shopping-cart}}
\def\faFolder{\faicon{folder}}
\def\faFolderOpen{\faicon{folder-open}}
\def\faArrowsV{\faicon{arrows-v}}
\def\faArrowsH{\faicon{arrows-h}}
\def\faBarChart{\faicon{bar-chart}}
\def\faTwitterSquare{\faicon{twitter-square}}
\def\faFacebookSquare{\faicon{facebook-square}}
\def\faCameraRetro{\faicon{camera-retro}}
\def\faKey{\faicon{key}}
\def\faCogs{\faicon{cogs}}
\def\faComments{\faicon{comments}}
\def\faThumbsOUp{\faicon{thumbs-o-up}}
\def\faThumbsODown{\faicon{thumbs-o-down}}
\def\faStarHalf{\faicon{star-half}}
\def\faHeartO{\faicon{heart-o}}
\def\faSignOut{\faicon{sign-out}}
\def\faLinkedinSquare{\faicon{linkedin-square}}
\def\faThumbTack{\faicon{thumb-tack}}
\def\faExternalLink{\faicon{external-link}}
\def\faSignIn{\faicon{sign-in}}
\def\faTrophy{\faicon{trophy}}
\def\faGithubSquare{\faicon{github-square}}
\def\faUpload{\faicon{upload}}
\def\faLemonO{\faicon{lemon-o}}
\def\faPhone{\faicon{phone}}
\def\faSquareO{\faicon{square-o}}
\def\faBookmarkO{\faicon{bookmark-o}}
\def\faPhoneSquare{\faicon{phone-square}}
\def\faTwitter{\faicon{twitter}}
\def\faFacebook{\faicon{facebook}}
\def\faGithub{\faicon{github}}
\def\faUnlock{\faicon{unlock}}
\def\faCreditCard{\faicon{credit-card}}
\def\faRss{\faicon{rss}}
\def\faHddO{\faicon{hdd-o}}
\def\faBullhorn{\faicon{bullhorn}}
\def\faBell{\faicon{bell}}
\def\faCertificate{\faicon{certificate}}
\def\faHandORight{\faicon{hand-o-right}}
\def\faHandOLeft{\faicon{hand-o-left}}
\def\faHandOUp{\faicon{hand-o-up}}
\def\faHandODown{\faicon{hand-o-down}}
\def\faArrowCircleLeft{\faicon{arrow-circle-left}}
\def\faArrowCircleRight{\faicon{arrow-circle-right}}
\def\faArrowCircleUp{\faicon{arrow-circle-up}}
\def\faArrowCircleDown{\faicon{arrow-circle-down}}
\def\faGlobe{\faicon{globe}}
\def\faWrench{\faicon{wrench}}
\def\faTasks{\faicon{tasks}}
\def\faFilter{\faicon{filter}}
\def\faBriefcase{\faicon{briefcase}}
\def\faArrowsAlt{\faicon{arrows-alt}}
\def\faUsers{\faicon{users}}
\def\faLink{\faicon{link}}
\def\faCloud{\faicon{cloud}}
\def\faFlask{\faicon{flask}}
\def\faScissors{\faicon{scissors}}
\def\faFilesO{\faicon{files-o}}
\def\faPaperclip{\faicon{paperclip}}
\def\faFloppyO{\faicon{floppy-o}}
\def\faSquare{\faicon{square}}
\def\faBars{\faicon{bars}}
\def\faListUl{\faicon{list-ul}}
\def\faListOl{\faicon{list-ol}}
\def\faStrikethrough{\faicon{strikethrough}}
\def\faUnderline{\faicon{underline}}
\def\faTable{\faicon{table}}
\def\faMagic{\faicon{magic}}
\def\faTruck{\faicon{truck}}
\def\faPinterest{\faicon{pinterest}}
\def\faPinterestSquare{\faicon{pinterest-square}}
\def\faGooglePlusSquare{\faicon{google-plus-square}}
\def\faGooglePlus{\faicon{google-plus}}
\def\faMoney{\faicon{money}}
\def\faCaretDown{\faicon{caret-down}}
\def\faCaretUp{\faicon{caret-up}}
\def\faCaretLeft{\faicon{caret-left}}
\def\faCaretRight{\faicon{caret-right}}
\def\faColumns{\faicon{columns}}
\def\faSort{\faicon{sort}}
\def\faSortDesc{\faicon{sort-desc}}
\def\faSortAsc{\faicon{sort-asc}}
\def\faEnvelope{\faicon{envelope}}
\def\faLinkedin{\faicon{linkedin}}
\def\faUndo{\faicon{undo}}
\def\faGavel{\faicon{gavel}}
\def\faTachometer{\faicon{tachometer}}
\def\faCommentO{\faicon{comment-o}}
\def\faCommentsO{\faicon{comments-o}}
\def\faBolt{\faicon{bolt}}
\def\faSitemap{\faicon{sitemap}}
\def\faUmbrella{\faicon{umbrella}}
\def\faClipboard{\faicon{clipboard}}
\def\faLightbulbO{\faicon{lightbulb-o}}
\def\faExchange{\faicon{exchange}}
\def\faCloudDownload{\faicon{cloud-download}}
\def\faCloudUpload{\faicon{cloud-upload}}
\def\faUserMd{\faicon{user-md}}
\def\faStethoscope{\faicon{stethoscope}}
\def\faSuitcase{\faicon{suitcase}}
\def\faBellO{\faicon{bell-o}}
\def\faCoffee{\faicon{coffee}}
\def\faCutlery{\faicon{cutlery}}
\def\faFileTextO{\faicon{file-text-o}}
\def\faBuildingO{\faicon{building-o}}
\def\faHospitalO{\faicon{hospital-o}}
\def\faAmbulance{\faicon{ambulance}}
\def\faMedkit{\faicon{medkit}}
\def\faFighterJet{\faicon{fighter-jet}}
\def\faBeer{\faicon{beer}}
\def\faHSquare{\faicon{h-square}}
\def\faPlusSquare{\faicon{plus-square}}
\def\faAngleDoubleLeft{\faicon{angle-double-left}}
\def\faAngleDoubleRight{\faicon{angle-double-right}}
\def\faAngleDoubleUp{\faicon{angle-double-up}}
\def\faAngleDoubleDown{\faicon{angle-double-down}}
\def\faAngleLeft{\faicon{angle-left}}
\def\faAngleRight{\faicon{angle-right}}
\def\faAngleUp{\faicon{angle-up}}
\def\faAngleDown{\faicon{angle-down}}
\def\faDesktop{\faicon{desktop}}
\def\faLaptop{\faicon{laptop}}
\def\faTablet{\faicon{tablet}}
\def\faMobile{\faicon{mobile}}
\def\faCircleO{\faicon{circle-o}}
\def\faQuoteLeft{\faicon{quote-left}}
\def\faQuoteRight{\faicon{quote-right}}
\def\faSpinner{\faicon{spinner}}
\def\faCircle{\faicon{circle}}
\def\faReply{\faicon{reply}}
\def\faGithubAlt{\faicon{github-alt}}
\def\faFolderO{\faicon{folder-o}}
\def\faFolderOpenO{\faicon{folder-open-o}}
\def\faSmileO{\faicon{smile-o}}
\def\faFrownO{\faicon{frown-o}}
\def\faMehO{\faicon{meh-o}}
\def\faGamepad{\faicon{gamepad}}
\def\faKeyboardO{\faicon{keyboard-o}}
\def\faFlagO{\faicon{flag-o}}
\def\faFlagCheckered{\faicon{flag-checkered}}
\def\faTerminal{\faicon{terminal}}
\def\faCode{\faicon{code}}
\def\faReplyAll{\faicon{reply-all}}
\def\faStarHalfO{\faicon{star-half-o}}
\def\faLocationArrow{\faicon{location-arrow}}
\def\faCrop{\faicon{crop}}
\def\faCodeFork{\faicon{code-fork}}
\def\faChainBroken{\faicon{chain-broken}}
\def\faQuestion{\faicon{question}}
\def\faInfo{\faicon{info}}
\def\faExclamation{\faicon{exclamation}}
\def\faSuperscript{\faicon{superscript}}
\def\faSubscript{\faicon{subscript}}
\def\faEraser{\faicon{eraser}}
\def\faPuzzlePiece{\faicon{puzzle-piece}}
\def\faMicrophone{\faicon{microphone}}
\def\faMicrophoneSlash{\faicon{microphone-slash}}
\def\faShield{\faicon{shield}}
\def\faCalendarO{\faicon{calendar-o}}
\def\faFireExtinguisher{\faicon{fire-extinguisher}}
\def\faRocket{\faicon{rocket}}
\def\faMaxcdn{\faicon{maxcdn}}
\def\faChevronCircleLeft{\faicon{chevron-circle-left}}
\def\faChevronCircleRight{\faicon{chevron-circle-right}}
\def\faChevronCircleUp{\faicon{chevron-circle-up}}
\def\faChevronCircleDown{\faicon{chevron-circle-down}}
\def\faHtml5{\faicon{html5}}
\def\faCss3{\faicon{css3}}
\def\faAnchor{\faicon{anchor}}
\def\faUnlockAlt{\faicon{unlock-alt}}
\def\faBullseye{\faicon{bullseye}}
\def\faEllipsisH{\faicon{ellipsis-h}}
\def\faEllipsisV{\faicon{ellipsis-v}}
\def\faRssSquare{\faicon{rss-square}}
\def\faPlayCircle{\faicon{play-circle}}
\def\faTicket{\faicon{ticket}}
\def\faMinusSquare{\faicon{minus-square}}
\def\faMinusSquareO{\faicon{minus-square-o}}
\def\faLevelUp{\faicon{level-up}}
\def\faLevelDown{\faicon{level-down}}
\def\faCheckSquare{\faicon{check-square}}
\def\faPencilSquare{\faicon{pencil-square}}
\def\faExternalLinkSquare{\faicon{external-link-square}}
\def\faShareSquare{\faicon{share-square}}
\def\faCompass{\faicon{compass}}
\def\faCaretSquareODown{\faicon{caret-square-o-down}}
\def\faCaretSquareOUp{\faicon{caret-square-o-up}}
\def\faCaretSquareORight{\faicon{caret-square-o-right}}
\def\faEur{\faicon{eur}}
\def\faGbp{\faicon{gbp}}
\def\faUsd{\faicon{usd}}
\def\faInr{\faicon{inr}}
\def\faJpy{\faicon{jpy}}
\def\faRub{\faicon{rub}}
\def\faKrw{\faicon{krw}}
\def\faBtc{\faicon{btc}}
\def\faFile{\faicon{file}}
\def\faFileText{\faicon{file-text}}
\def\faSortAlphaAsc{\faicon{sort-alpha-asc}}
\def\faSortAlphaDesc{\faicon{sort-alpha-desc}}
\def\faSortAmountAsc{\faicon{sort-amount-asc}}
\def\faSortAmountDesc{\faicon{sort-amount-desc}}
\def\faSortNumericAsc{\faicon{sort-numeric-asc}}
\def\faSortNumericDesc{\faicon{sort-numeric-desc}}
\def\faThumbsUp{\faicon{thumbs-up}}
\def\faThumbsDown{\faicon{thumbs-down}}
\def\faYoutubeSquare{\faicon{youtube-square}}
\def\faYoutube{\faicon{youtube}}
\def\faXing{\faicon{xing}}
\def\faXingSquare{\faicon{xing-square}}
\def\faYoutubePlay{\faicon{youtube-play}}
\def\faDropbox{\faicon{dropbox}}
\def\faStackOverflow{\faicon{stack-overflow}}
\def\faInstagram{\faicon{instagram}}
\def\faFlickr{\faicon{flickr}}
\def\faAdn{\faicon{adn}}
\def\faBitbucket{\faicon{bitbucket}}
\def\faBitbucketSquare{\faicon{bitbucket-square}}
\def\faTumblr{\faicon{tumblr}}
\def\faTumblrSquare{\faicon{tumblr-square}}
\def\faLongArrowDown{\faicon{long-arrow-down}}
\def\faLongArrowUp{\faicon{long-arrow-up}}
\def\faLongArrowLeft{\faicon{long-arrow-left}}
\def\faLongArrowRight{\faicon{long-arrow-right}}
\def\faApple{\faicon{apple}}
\def\faWindows{\faicon{windows}}
\def\faAndroid{\faicon{android}}
\def\faLinux{\faicon{linux}}
\def\faDribbble{\faicon{dribbble}}
\def\faSkype{\faicon{skype}}
\def\faFoursquare{\faicon{foursquare}}
\def\faTrello{\faicon{trello}}
\def\faFemale{\faicon{female}}
\def\faMale{\faicon{male}}
\def\faGratipay{\faicon{gratipay}}
\def\faSunO{\faicon{sun-o}}
\def\faMoonO{\faicon{moon-o}}
\def\faArchive{\faicon{archive}}
\def\faBug{\faicon{bug}}
\def\faVk{\faicon{vk}}
\def\faWeibo{\faicon{weibo}}
\def\faRenren{\faicon{renren}}
\def\faPagelines{\faicon{pagelines}}
\def\faStackExchange{\faicon{stack-exchange}}
\def\faArrowCircleORight{\faicon{arrow-circle-o-right}}
\def\faArrowCircleOLeft{\faicon{arrow-circle-o-left}}
\def\faCaretSquareOLeft{\faicon{caret-square-o-left}}
\def\faDotCircleO{\faicon{dot-circle-o}}
\def\faWheelchair{\faicon{wheelchair}}
\def\faVimeoSquare{\faicon{vimeo-square}}
\def\faTry{\faicon{try}}
\def\faPlusSquareO{\faicon{plus-square-o}}
\def\faSpaceShuttle{\faicon{space-shuttle}}
\def\faSlack{\faicon{slack}}
\def\faEnvelopeSquare{\faicon{envelope-square}}
\def\faWordpress{\faicon{wordpress}}
\def\faOpenid{\faicon{openid}}
\def\faUniversity{\faicon{university}}
\def\faGraduationCap{\faicon{graduation-cap}}
\def\faYahoo{\faicon{yahoo}}
\def\faGoogle{\faicon{google}}
\def\faReddit{\faicon{reddit}}
\def\faRedditSquare{\faicon{reddit-square}}
\def\faStumbleuponCircle{\faicon{stumbleupon-circle}}
\def\faStumbleupon{\faicon{stumbleupon}}
\def\faDelicious{\faicon{delicious}}
\def\faDigg{\faicon{digg}}
\def\faPiedPiperPp{\faicon{pied-piper-pp}}
\def\faPiedPiperAlt{\faicon{pied-piper-alt}}
\def\faDrupal{\faicon{drupal}}
\def\faJoomla{\faicon{joomla}}
\def\faLanguage{\faicon{language}}
\def\faFax{\faicon{fax}}
\def\faBuilding{\faicon{building}}
\def\faChild{\faicon{child}}
\def\faPaw{\faicon{paw}}
\def\faSpoon{\faicon{spoon}}
\def\faCube{\faicon{cube}}
\def\faCubes{\faicon{cubes}}
\def\faBehance{\faicon{behance}}
\def\faBehanceSquare{\faicon{behance-square}}
\def\faSteam{\faicon{steam}}
\def\faSteamSquare{\faicon{steam-square}}
\def\faRecycle{\faicon{recycle}}
\def\faCar{\faicon{car}}
\def\faTaxi{\faicon{taxi}}
\def\faTree{\faicon{tree}}
\def\faSpotify{\faicon{spotify}}
\def\faDeviantart{\faicon{deviantart}}
\def\faSoundcloud{\faicon{soundcloud}}
\def\faDatabase{\faicon{database}}
\def\faFilePdfO{\faicon{file-pdf-o}}
\def\faFileWordO{\faicon{file-word-o}}
\def\faFileExcelO{\faicon{file-excel-o}}
\def\faFilePowerpointO{\faicon{file-powerpoint-o}}
\def\faFileImageO{\faicon{file-image-o}}
\def\faFileArchiveO{\faicon{file-archive-o}}
\def\faFileAudioO{\faicon{file-audio-o}}
\def\faFileVideoO{\faicon{file-video-o}}
\def\faFileCodeO{\faicon{file-code-o}}
\def\faVine{\faicon{vine}}
\def\faCodepen{\faicon{codepen}}
\def\faJsfiddle{\faicon{jsfiddle}}
\def\faLifeRing{\faicon{life-ring}}
\def\faCircleONotch{\faicon{circle-o-notch}}
\def\faRebel{\faicon{rebel}}
\def\faEmpire{\faicon{empire}}
\def\faGitSquare{\faicon{git-square}}
\def\faGit{\faicon{git}}
\def\faHackerNews{\faicon{hacker-news}}
\def\faTencentWeibo{\faicon{tencent-weibo}}
\def\faQq{\faicon{qq}}
\def\faWeixin{\faicon{weixin}}
\def\faPaperPlane{\faicon{paper-plane}}
\def\faPaperPlaneO{\faicon{paper-plane-o}}
\def\faHistory{\faicon{history}}
\def\faCircleThin{\faicon{circle-thin}}
\def\faHeader{\faicon{header}}
\def\faParagraph{\faicon{paragraph}}
\def\faSliders{\faicon{sliders}}
\def\faShareAlt{\faicon{share-alt}}
\def\faShareAltSquare{\faicon{share-alt-square}}
\def\faBomb{\faicon{bomb}}
\def\faFutbolO{\faicon{futbol-o}}
\def\faTty{\faicon{tty}}
\def\faBinoculars{\faicon{binoculars}}
\def\faPlug{\faicon{plug}}
\def\faSlideshare{\faicon{slideshare}}
\def\faTwitch{\faicon{twitch}}
\def\faYelp{\faicon{yelp}}
\def\faNewspaperO{\faicon{newspaper-o}}
\def\faWifi{\faicon{wifi}}
\def\faCalculator{\faicon{calculator}}
\def\faPaypal{\faicon{paypal}}
\def\faGoogleWallet{\faicon{google-wallet}}
\def\faCcVisa{\faicon{cc-visa}}
\def\faCcMastercard{\faicon{cc-mastercard}}
\def\faCcDiscover{\faicon{cc-discover}}
\def\faCcAmex{\faicon{cc-amex}}
\def\faCcPaypal{\faicon{cc-paypal}}
\def\faCcStripe{\faicon{cc-stripe}}
\def\faBellSlash{\faicon{bell-slash}}
\def\faBellSlashO{\faicon{bell-slash-o}}
\def\faTrash{\faicon{trash}}
\def\faCopyright{\faicon{copyright}}
\def\faAt{\faicon{at}}
\def\faEyedropper{\faicon{eyedropper}}
\def\faPaintBrush{\faicon{paint-brush}}
\def\faBirthdayCake{\faicon{birthday-cake}}
\def\faAreaChart{\faicon{area-chart}}
\def\faPieChart{\faicon{pie-chart}}
\def\faLineChart{\faicon{line-chart}}
\def\faLastfm{\faicon{lastfm}}
\def\faLastfmSquare{\faicon{lastfm-square}}
\def\faToggleOff{\faicon{toggle-off}}
\def\faToggleOn{\faicon{toggle-on}}
\def\faBicycle{\faicon{bicycle}}
\def\faBus{\faicon{bus}}
\def\faIoxhost{\faicon{ioxhost}}
\def\faAngellist{\faicon{angellist}}
\def\faCc{\faicon{cc}}
\def\faIls{\faicon{ils}}
\def\faMeanpath{\faicon{meanpath}}
\def\faBuysellads{\faicon{buysellads}}
\def\faConnectdevelop{\faicon{connectdevelop}}
\def\faDashcube{\faicon{dashcube}}
\def\faForumbee{\faicon{forumbee}}
\def\faLeanpub{\faicon{leanpub}}
\def\faSellsy{\faicon{sellsy}}
\def\faShirtsinbulk{\faicon{shirtsinbulk}}
\def\faSimplybuilt{\faicon{simplybuilt}}
\def\faSkyatlas{\faicon{skyatlas}}
\def\faCartPlus{\faicon{cart-plus}}
\def\faCartArrowDown{\faicon{cart-arrow-down}}
\def\faDiamond{\faicon{diamond}}
\def\faShip{\faicon{ship}}
\def\faUserSecret{\faicon{user-secret}}
\def\faMotorcycle{\faicon{motorcycle}}
\def\faStreetView{\faicon{street-view}}
\def\faHeartbeat{\faicon{heartbeat}}
\def\faVenus{\faicon{venus}}
\def\faMars{\faicon{mars}}
\def\faMercury{\faicon{mercury}}
\def\faTransgender{\faicon{transgender}}
\def\faTransgenderAlt{\faicon{transgender-alt}}
\def\faVenusDouble{\faicon{venus-double}}
\def\faMarsDouble{\faicon{mars-double}}
\def\faVenusMars{\faicon{venus-mars}}
\def\faMarsStroke{\faicon{mars-stroke}}
\def\faMarsStrokeV{\faicon{mars-stroke-v}}
\def\faMarsStrokeH{\faicon{mars-stroke-h}}
\def\faNeuter{\faicon{neuter}}
\def\faGenderless{\faicon{genderless}}
\def\faFacebookOfficial{\faicon{facebook-official}}
\def\faPinterestP{\faicon{pinterest-p}}
\def\faWhatsapp{\faicon{whatsapp}}
\def\faServer{\faicon{server}}
\def\faUserPlus{\faicon{user-plus}}
\def\faUserTimes{\faicon{user-times}}
\def\faBed{\faicon{bed}}
\def\faViacoin{\faicon{viacoin}}
\def\faTrain{\faicon{train}}
\def\faSubway{\faicon{subway}}
\def\faMedium{\faicon{medium}}
\def\faYCombinator{\faicon{y-combinator}}
\def\faOptinMonster{\faicon{optin-monster}}
\def\faOpencart{\faicon{opencart}}
\def\faExpeditedssl{\faicon{expeditedssl}}
\def\faBatteryFull{\faicon{battery-full}}
\def\faBatteryThreeQuarters{\faicon{battery-three-quarters}}
\def\faBatteryHalf{\faicon{battery-half}}
\def\faBatteryQuarter{\faicon{battery-quarter}}
\def\faBatteryEmpty{\faicon{battery-empty}}
\def\faMousePointer{\faicon{mouse-pointer}}
\def\faICursor{\faicon{i-cursor}}
\def\faObjectGroup{\faicon{object-group}}
\def\faObjectUngroup{\faicon{object-ungroup}}
\def\faStickyNote{\faicon{sticky-note}}
\def\faStickyNoteO{\faicon{sticky-note-o}}
\def\faCcJcb{\faicon{cc-jcb}}
\def\faCcDinersClub{\faicon{cc-diners-club}}
\def\faClone{\faicon{clone}}
\def\faBalanceScale{\faicon{balance-scale}}
\def\faHourglassO{\faicon{hourglass-o}}
\def\faHourglassStart{\faicon{hourglass-start}}
\def\faHourglassHalf{\faicon{hourglass-half}}
\def\faHourglassEnd{\faicon{hourglass-end}}
\def\faHourglass{\faicon{hourglass}}
\def\faHandRockO{\faicon{hand-rock-o}}
\def\faHandPaperO{\faicon{hand-paper-o}}
\def\faHandScissorsO{\faicon{hand-scissors-o}}
\def\faHandLizardO{\faicon{hand-lizard-o}}
\def\faHandSpockO{\faicon{hand-spock-o}}
\def\faHandPointerO{\faicon{hand-pointer-o}}
\def\faHandPeaceO{\faicon{hand-peace-o}}
\def\faTrademark{\faicon{trademark}}
\def\faRegistered{\faicon{registered}}
\def\faCreativeCommons{\faicon{creative-commons}}
\def\faGg{\faicon{gg}}
\def\faGgCircle{\faicon{gg-circle}}
\def\faTripadvisor{\faicon{tripadvisor}}
\def\faOdnoklassniki{\faicon{odnoklassniki}}
\def\faOdnoklassnikiSquare{\faicon{odnoklassniki-square}}
\def\faGetPocket{\faicon{get-pocket}}
\def\faWikipediaW{\faicon{wikipedia-w}}
\def\faSafari{\faicon{safari}}
\def\faChrome{\faicon{chrome}}
\def\faFirefox{\faicon{firefox}}
\def\faOpera{\faicon{opera}}
\def\faInternetExplorer{\faicon{internet-explorer}}
\def\faTelevision{\faicon{television}}
\def\faContao{\faicon{contao}}
\def\fa500Px{\faicon{500px}}
\def\faAmazon{\faicon{amazon}}
\def\faCalendarPlusO{\faicon{calendar-plus-o}}
\def\faCalendarMinusO{\faicon{calendar-minus-o}}
\def\faCalendarTimesO{\faicon{calendar-times-o}}
\def\faCalendarCheckO{\faicon{calendar-check-o}}
\def\faIndustry{\faicon{industry}}
\def\faMapPin{\faicon{map-pin}}
\def\faMapSigns{\faicon{map-signs}}
\def\faMapO{\faicon{map-o}}
\def\faMap{\faicon{map}}
\def\faCommenting{\faicon{commenting}}
\def\faCommentingO{\faicon{commenting-o}}
\def\faHouzz{\faicon{houzz}}
\def\faVimeo{\faicon{vimeo}}
\def\faBlackTie{\faicon{black-tie}}
\def\faFonticons{\faicon{fonticons}}
\def\faRedditAlien{\faicon{reddit-alien}}
\def\faEdge{\faicon{edge}}
\def\faCreditCardAlt{\faicon{credit-card-alt}}
\def\faCodiepie{\faicon{codiepie}}
\def\faModx{\faicon{modx}}
\def\faFortAwesome{\faicon{fort-awesome}}
\def\faUsb{\faicon{usb}}
\def\faProductHunt{\faicon{product-hunt}}
\def\faMixcloud{\faicon{mixcloud}}
\def\faScribd{\faicon{scribd}}
\def\faPauseCircle{\faicon{pause-circle}}
\def\faPauseCircleO{\faicon{pause-circle-o}}
\def\faStopCircle{\faicon{stop-circle}}
\def\faStopCircleO{\faicon{stop-circle-o}}
\def\faShoppingBag{\faicon{shopping-bag}}
\def\faShoppingBasket{\faicon{shopping-basket}}
\def\faHashtag{\faicon{hashtag}}
\def\faBluetooth{\faicon{bluetooth}}
\def\faBluetoothB{\faicon{bluetooth-b}}
\def\faPercent{\faicon{percent}}
\def\faGitlab{\faicon{gitlab}}
\def\faWpbeginner{\faicon{wpbeginner}}
\def\faWpforms{\faicon{wpforms}}
\def\faEnvira{\faicon{envira}}
\def\faUniversalAccess{\faicon{universal-access}}
\def\faWheelchairAlt{\faicon{wheelchair-alt}}
\def\faQuestionCircleO{\faicon{question-circle-o}}
\def\faBlind{\faicon{blind}}
\def\faAudioDescription{\faicon{audio-description}}
\def\faVolumeControlPhone{\faicon{volume-control-phone}}
\def\faBraille{\faicon{braille}}
\def\faAssistiveListeningSystems{\faicon{assistive-listening-systems}}
\def\faAmericanSignLanguageInterpreting{\faicon{american-sign-language-interpreting}}
\def\faDeaf{\faicon{deaf}}
\def\faGlide{\faicon{glide}}
\def\faGlideG{\faicon{glide-g}}
\def\faSignLanguage{\faicon{sign-language}}
\def\faLowVision{\faicon{low-vision}}
\def\faViadeo{\faicon{viadeo}}
\def\faViadeoSquare{\faicon{viadeo-square}}
\def\faSnapchat{\faicon{snapchat}}
\def\faSnapchatGhost{\faicon{snapchat-ghost}}
\def\faSnapchatSquare{\faicon{snapchat-square}}
\def\faPiedPiper{\faicon{pied-piper}}
\def\faFirstOrder{\faicon{first-order}}
\def\faYoast{\faicon{yoast}}
\def\faThemeisle{\faicon{themeisle}}
\def\faGooglePlusOfficial{\faicon{google-plus-official}}
\def\faFontAwesome{\faicon{font-awesome}}
% aliases
\def\faCny{\faicon{cny}}\expandafter\def\csname faicon@cny\endcsname{\faicon{jpy}}
\def\faYCombinatorSquare{\faicon{y-combinator-square}}\expandafter\def\csname faicon@y-combinator-square\endcsname{\faicon{hacker-news}}
\def\faCab{\faicon{cab}}\expandafter\def\csname faicon@cab\endcsname{\faicon{taxi}}
\def\faToggleUp{\faicon{toggle-up}}\expandafter\def\csname faicon@toggle-up\endcsname{\faicon{caret-square-o-up}}
\def\faLifeBuoy{\faicon{life-buoy}}\expandafter\def\csname faicon@life-buoy\endcsname{\faicon{life-ring}}
\def\faFileZipO{\faicon{file-zip-o}}\expandafter\def\csname faicon@file-zip-o\endcsname{\faicon{file-archive-o}}
\def\faBitcoin{\faicon{bitcoin}}\expandafter\def\csname faicon@bitcoin\endcsname{\faicon{btc}}
\def\faAutomobile{\faicon{automobile}}\expandafter\def\csname faicon@automobile\endcsname{\faicon{car}}
\def\faPaste{\faicon{paste}}\expandafter\def\csname faicon@paste\endcsname{\faicon{clipboard}}
\def\faResistance{\faicon{resistance}}\expandafter\def\csname faicon@resistance\endcsname{\faicon{rebel}}
\def\faCopy{\faicon{copy}}\expandafter\def\csname faicon@copy\endcsname{\faicon{files-o}}
\def\faIntersex{\faicon{intersex}}\expandafter\def\csname faicon@intersex\endcsname{\faicon{transgender}}
\def\faHardOfHearing{\faicon{hard-of-hearing}}\expandafter\def\csname faicon@hard-of-hearing\endcsname{\faicon{deaf}}
\def\faMailReply{\faicon{mail-reply}}\expandafter\def\csname faicon@mail-reply\endcsname{\faicon{reply}}
\def\faSortDown{\faicon{sort-down}}\expandafter\def\csname faicon@sort-down\endcsname{\faicon{sort-desc}}
\def\faGe{\faicon{ge}}\expandafter\def\csname faicon@ge\endcsname{\faicon{empire}}
\def\faBattery2{\faicon{battery-2}}\expandafter\def\csname faicon@battery-2\endcsname{\faicon{battery-half}}
\def\faHandStopO{\faicon{hand-stop-o}}\expandafter\def\csname faicon@hand-stop-o\endcsname{\faicon{hand-paper-o}}
\def\faGroup{\faicon{group}}\expandafter\def\csname faicon@group\endcsname{\faicon{users}}
\def\faRotateRight{\faicon{rotate-right}}\expandafter\def\csname faicon@rotate-right\endcsname{\faicon{repeat}}
\def\faWon{\faicon{won}}\expandafter\def\csname faicon@won\endcsname{\faicon{krw}}
\def\faFa{\faicon{fa}}\expandafter\def\csname faicon@fa\endcsname{\faicon{font-awesome}}
\def\faHourglass3{\faicon{hourglass-3}}\expandafter\def\csname faicon@hourglass-3\endcsname{\faicon{hourglass-end}}
\def\faStarHalfEmpty{\faicon{star-half-empty}}\expandafter\def\csname faicon@star-half-empty\endcsname{\faicon{star-half-o}}
\def\faCut{\faicon{cut}}\expandafter\def\csname faicon@cut\endcsname{\faicon{scissors}}
\def\faToggleDown{\faicon{toggle-down}}\expandafter\def\csname faicon@toggle-down\endcsname{\faicon{caret-square-o-down}}
\def\faGooglePlusCircle{\faicon{google-plus-circle}}\expandafter\def\csname faicon@google-plus-circle\endcsname{\faicon{google-plus-official}}
\def\faSheqel{\faicon{sheqel}}\expandafter\def\csname faicon@sheqel\endcsname{\faicon{ils}}
\def\faDashboard{\faicon{dashboard}}\expandafter\def\csname faicon@dashboard\endcsname{\faicon{tachometer}}
\def\faSend{\faicon{send}}\expandafter\def\csname faicon@send\endcsname{\faicon{paper-plane}}
\def\faYc{\faicon{yc}}\expandafter\def\csname faicon@yc\endcsname{\faicon{y-combinator}}
\def\faToggleLeft{\faicon{toggle-left}}\expandafter\def\csname faicon@toggle-left\endcsname{\faicon{caret-square-o-left}}
\def\faWarning{\faicon{warning}}\expandafter\def\csname faicon@warning\endcsname{\faicon{exclamation-triangle}}
\def\faImage{\faicon{image}}\expandafter\def\csname faicon@image\endcsname{\faicon{picture-o}}
\def\faInstitution{\faicon{institution}}\expandafter\def\csname faicon@institution\endcsname{\faicon{university}}
\def\faFileMovieO{\faicon{file-movie-o}}\expandafter\def\csname faicon@file-movie-o\endcsname{\faicon{file-video-o}}
\def\faPhoto{\faicon{photo}}\expandafter\def\csname faicon@photo\endcsname{\faicon{picture-o}}
\def\faFileSoundO{\faicon{file-sound-o}}\expandafter\def\csname faicon@file-sound-o\endcsname{\faicon{file-audio-o}}
\def\faMortarBoard{\faicon{mortar-board}}\expandafter\def\csname faicon@mortar-board\endcsname{\faicon{graduation-cap}}
\def\faGittip{\faicon{gittip}}\expandafter\def\csname faicon@gittip\endcsname{\faicon{gratipay}}
\def\faHourglass2{\faicon{hourglass-2}}\expandafter\def\csname faicon@hourglass-2\endcsname{\faicon{hourglass-half}}
\def\faSupport{\faicon{support}}\expandafter\def\csname faicon@support\endcsname{\faicon{life-ring}}
\def\faEdit{\faicon{edit}}\expandafter\def\csname faicon@edit\endcsname{\faicon{pencil-square-o}}
\def\faHotel{\faicon{hotel}}\expandafter\def\csname faicon@hotel\endcsname{\faicon{bed}}
\def\faSoccerBallO{\faicon{soccer-ball-o}}\expandafter\def\csname faicon@soccer-ball-o\endcsname{\faicon{futbol-o}}
\def\faFilePictureO{\faicon{file-picture-o}}\expandafter\def\csname faicon@file-picture-o\endcsname{\faicon{file-image-o}}
\def\faClose{\faicon{close}}\expandafter\def\csname faicon@close\endcsname{\faicon{times}}
\def\faYcSquare{\faicon{yc-square}}\expandafter\def\csname faicon@yc-square\endcsname{\faicon{hacker-news}}
\def\faShekel{\faicon{shekel}}\expandafter\def\csname faicon@shekel\endcsname{\faicon{ils}}
\def\faDollar{\faicon{dollar}}\expandafter\def\csname faicon@dollar\endcsname{\faicon{usd}}
\def\faUnsorted{\faicon{unsorted}}\expandafter\def\csname faicon@unsorted\endcsname{\faicon{sort}}
\def\faReorder{\faicon{reorder}}\expandafter\def\csname faicon@reorder\endcsname{\faicon{bars}}
\def\faBattery3{\faicon{battery-3}}\expandafter\def\csname faicon@battery-3\endcsname{\faicon{battery-three-quarters}}
\def\faRupee{\faicon{rupee}}\expandafter\def\csname faicon@rupee\endcsname{\faicon{inr}}
\def\faRouble{\faicon{rouble}}\expandafter\def\csname faicon@rouble\endcsname{\faicon{rub}}
\def\faHourglass1{\faicon{hourglass-1}}\expandafter\def\csname faicon@hourglass-1\endcsname{\faicon{hourglass-start}}
\def\faAslInterpreting{\faicon{asl-interpreting}}\expandafter\def\csname faicon@asl-interpreting\endcsname{\faicon{american-sign-language-interpreting}}
\def\faTv{\faicon{tv}}\expandafter\def\csname faicon@tv\endcsname{\faicon{television}}
\def\faSave{\faicon{save}}\expandafter\def\csname faicon@save\endcsname{\faicon{floppy-o}}
\def\faToggleRight{\faicon{toggle-right}}\expandafter\def\csname faicon@toggle-right\endcsname{\faicon{caret-square-o-right}}
\def\faDedent{\faicon{dedent}}\expandafter\def\csname faicon@dedent\endcsname{\faicon{outdent}}
\def\faGear{\faicon{gear}}\expandafter\def\csname faicon@gear\endcsname{\faicon{cog}}
\def\faLegal{\faicon{legal}}\expandafter\def\csname faicon@legal\endcsname{\faicon{gavel}}
\def\faWechat{\faicon{wechat}}\expandafter\def\csname faicon@wechat\endcsname{\faicon{weixin}}
\def\faFacebookF{\faicon{facebook-f}}\expandafter\def\csname faicon@facebook-f\endcsname{\faicon{facebook}}
\def\faFeed{\faicon{feed}}\expandafter\def\csname faicon@feed\endcsname{\faicon{rss}}
\def\faBank{\faicon{bank}}\expandafter\def\csname faicon@bank\endcsname{\faicon{university}}
\def\faTurkishLira{\faicon{turkish-lira}}\expandafter\def\csname faicon@turkish-lira\endcsname{\faicon{try}}
\def\faUnlink{\faicon{unlink}}\expandafter\def\csname faicon@unlink\endcsname{\faicon{chain-broken}}
\def\faChain{\faicon{chain}}\expandafter\def\csname faicon@chain\endcsname{\faicon{link}}
\def\faGears{\faicon{gears}}\expandafter\def\csname faicon@gears\endcsname{\faicon{cogs}}
\def\faRmb{\faicon{rmb}}\expandafter\def\csname faicon@rmb\endcsname{\faicon{jpy}}
\def\faBattery1{\faicon{battery-1}}\expandafter\def\csname faicon@battery-1\endcsname{\faicon{battery-quarter}}
\def\faLifeBouy{\faicon{life-bouy}}\expandafter\def\csname faicon@life-bouy\endcsname{\faicon{life-ring}}
\def\faYen{\faicon{yen}}\expandafter\def\csname faicon@yen\endcsname{\faicon{jpy}}
\def\faBattery4{\faicon{battery-4}}\expandafter\def\csname faicon@battery-4\endcsname{\faicon{battery-full}}
\def\faBattery0{\faicon{battery-0}}\expandafter\def\csname faicon@battery-0\endcsname{\faicon{battery-empty}}
\def\faHandGrabO{\faicon{hand-grab-o}}\expandafter\def\csname faicon@hand-grab-o\endcsname{\faicon{hand-rock-o}}
\def\faMailReplyAll{\faicon{mail-reply-all}}\expandafter\def\csname faicon@mail-reply-all\endcsname{\faicon{reply-all}}
\def\faMobilePhone{\faicon{mobile-phone}}\expandafter\def\csname faicon@mobile-phone\endcsname{\faicon{mobile}}
\def\faRotateLeft{\faicon{rotate-left}}\expandafter\def\csname faicon@rotate-left\endcsname{\faicon{undo}}
\def\faEuro{\faicon{euro}}\expandafter\def\csname faicon@euro\endcsname{\faicon{eur}}
\def\faRuble{\faicon{ruble}}\expandafter\def\csname faicon@ruble\endcsname{\faicon{rub}}
\def\faRa{\faicon{ra}}\expandafter\def\csname faicon@ra\endcsname{\faicon{rebel}}
\def\faStarHalfFull{\faicon{star-half-full}}\expandafter\def\csname faicon@star-half-full\endcsname{\faicon{star-half-o}}
\def\faSortUp{\faicon{sort-up}}\expandafter\def\csname faicon@sort-up\endcsname{\faicon{sort-asc}}
\def\faMailForward{\faicon{mail-forward}}\expandafter\def\csname faicon@mail-forward\endcsname{\faicon{share}}
\def\faSigning{\faicon{signing}}\expandafter\def\csname faicon@signing\endcsname{\faicon{sign-language}}
\def\faFlash{\faicon{flash}}\expandafter\def\csname faicon@flash\endcsname{\faicon{bolt}}
\def\faLifeSaver{\faicon{life-saver}}\expandafter\def\csname faicon@life-saver\endcsname{\faicon{life-ring}}
\def\faFilePhotoO{\faicon{file-photo-o}}\expandafter\def\csname faicon@file-photo-o\endcsname{\faicon{file-image-o}}
\def\faDeafness{\faicon{deafness}}\expandafter\def\csname faicon@deafness\endcsname{\faicon{deaf}}
\def\faBarChartO{\faicon{bar-chart-o}}\expandafter\def\csname faicon@bar-chart-o\endcsname{\faicon{bar-chart}}
\def\faSendO{\faicon{send-o}}\expandafter\def\csname faicon@send-o\endcsname{\faicon{paper-plane-o}}
\def\faNavicon{\faicon{navicon}}\expandafter\def\csname faicon@navicon\endcsname{\faicon{bars}}
\def\faRemove{\faicon{remove}}\expandafter\def\csname faicon@remove\endcsname{\faicon{times}}


==> fontawesomesymbols-pdftex.tex <==
%% start of file `fontawesomesymbols-pdftex.tex'.
\expandafter\def\csname faicon@info\endcsname{{\FAone\symbol{0}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FAone\symbol{1}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FAone\symbol{2}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FAone\symbol{3}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FAone\symbol{4}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FAone\symbol{5}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FAone\symbol{6}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FAone\symbol{7}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FAone\symbol{8}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FAone\symbol{9}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FAone\symbol{10}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FAone\symbol{11}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FAone\symbol{12}}}
\expandafter\def\csname faicon@try\endcsname{{\FAone\symbol{13}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FAone\symbol{14}}}
\expandafter\def\csname faicon@slack\endcsname{{\FAone\symbol{15}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FAone\symbol{16}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FAone\symbol{17}}}
\expandafter\def\csname faicon@openid\endcsname{{\FAone\symbol{18}}}
\expandafter\def\csname faicon@university\endcsname{{\FAone\symbol{19}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FAone\symbol{20}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FAone\symbol{21}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FAone\symbol{22}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FAone\symbol{23}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FAone\symbol{24}}}
\expandafter\def\csname faicon@digg\endcsname{{\FAone\symbol{25}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FAone\symbol{26}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FAone\symbol{27}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FAone\symbol{28}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FAone\symbol{29}}}
\expandafter\def\csname faicon@fax\endcsname{{\FAone\symbol{30}}}
\expandafter\def\csname faicon@building\endcsname{{\FAone\symbol{31}}}
\expandafter\def\csname faicon@child\endcsname{{\FAone\symbol{32}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FAone\symbol{33}}}
\expandafter\def\csname faicon@cube\endcsname{{\FAone\symbol{34}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FAone\symbol{35}}}
\expandafter\def\csname faicon@behance\endcsname{{\FAone\symbol{36}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FAone\symbol{37}}}
\expandafter\def\csname faicon@steam\endcsname{{\FAone\symbol{38}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FAone\symbol{39}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FAone\symbol{40}}}
\expandafter\def\csname faicon@car\endcsname{{\FAone\symbol{41}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FAone\symbol{42}}}
\expandafter\def\csname faicon@tree\endcsname{{\FAone\symbol{43}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FAone\symbol{44}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FAone\symbol{45}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FAone\symbol{46}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FAone\symbol{47}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FAone\symbol{48}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FAone\symbol{49}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FAone\symbol{50}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FAone\symbol{51}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FAone\symbol{52}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FAone\symbol{53}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FAone\symbol{54}}}
\expandafter\def\csname faicon@vine\endcsname{{\FAone\symbol{55}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FAone\symbol{56}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FAone\symbol{57}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FAone\symbol{58}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FAone\symbol{59}}}
\expandafter\def\csname faicon@git\endcsname{{\FAone\symbol{60}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FAone\symbol{61}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FAone\symbol{62}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FAone\symbol{63}}}
\expandafter\def\csname faicon@history\endcsname{{\FAone\symbol{64}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FAone\symbol{65}}}
\expandafter\def\csname faicon@header\endcsname{{\FAone\symbol{66}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FAone\symbol{67}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FAone\symbol{68}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FAone\symbol{69}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FAone\symbol{70}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FAone\symbol{71}}}
\expandafter\def\csname faicon@tty\endcsname{{\FAone\symbol{72}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FAone\symbol{73}}}
\expandafter\def\csname faicon@plug\endcsname{{\FAone\symbol{74}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FAone\symbol{75}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FAone\symbol{76}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FAone\symbol{77}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FAone\symbol{78}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FAone\symbol{79}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FAone\symbol{80}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FAone\symbol{81}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FAone\symbol{82}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FAone\symbol{83}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FAone\symbol{84}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FAone\symbol{85}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FAone\symbol{86}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FAone\symbol{87}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FAone\symbol{88}}}
\expandafter\def\csname faicon@trash\endcsname{{\FAone\symbol{89}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FAone\symbol{90}}}
\expandafter\def\csname faicon@at\endcsname{{\FAone\symbol{91}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FAone\symbol{92}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FAone\symbol{93}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FAone\symbol{94}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FAone\symbol{95}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FAone\symbol{96}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FAone\symbol{97}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FAone\symbol{98}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FAone\symbol{99}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FAone\symbol{100}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FAone\symbol{101}}}
\expandafter\def\csname faicon@bus\endcsname{{\FAone\symbol{102}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FAone\symbol{103}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FAone\symbol{104}}}
\expandafter\def\csname faicon@cc\endcsname{{\FAone\symbol{105}}}
\expandafter\def\csname faicon@ils\endcsname{{\FAone\symbol{106}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FAone\symbol{107}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FAone\symbol{108}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FAone\symbol{109}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FAone\symbol{110}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FAone\symbol{111}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FAone\symbol{112}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FAone\symbol{113}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FAone\symbol{114}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FAone\symbol{115}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FAone\symbol{116}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FAone\symbol{117}}}
\expandafter\def\csname faicon@ship\endcsname{{\FAone\symbol{118}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FAone\symbol{119}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FAone\symbol{120}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FAone\symbol{121}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FAone\symbol{122}}}
\expandafter\def\csname faicon@mars\endcsname{{\FAone\symbol{123}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FAone\symbol{124}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FAone\symbol{125}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FAone\symbol{126}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FAone\symbol{127}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FAone\symbol{128}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FAone\symbol{129}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FAone\symbol{130}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FAone\symbol{131}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FAone\symbol{132}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FAone\symbol{133}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FAone\symbol{134}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FAone\symbol{135}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FAone\symbol{136}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FAone\symbol{137}}}
\expandafter\def\csname faicon@server\endcsname{{\FAone\symbol{138}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FAone\symbol{139}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FAone\symbol{140}}}
\expandafter\def\csname faicon@bed\endcsname{{\FAone\symbol{141}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FAone\symbol{142}}}
\expandafter\def\csname faicon@train\endcsname{{\FAone\symbol{143}}}
\expandafter\def\csname faicon@subway\endcsname{{\FAone\symbol{144}}}
\expandafter\def\csname faicon@medium\endcsname{{\FAone\symbol{145}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FAone\symbol{146}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FAone\symbol{147}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FAone\symbol{148}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FAone\symbol{149}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FAone\symbol{150}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FAone\symbol{151}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FAone\symbol{152}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FAone\symbol{153}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FAone\symbol{154}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FAone\symbol{155}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FAone\symbol{156}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FAone\symbol{157}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FAone\symbol{158}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FAone\symbol{159}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FAone\symbol{160}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FAone\symbol{161}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FAone\symbol{162}}}
\expandafter\def\csname faicon@clone\endcsname{{\FAone\symbol{163}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FAone\symbol{164}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FAone\symbol{165}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FAone\symbol{166}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FAone\symbol{167}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FAone\symbol{168}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FAone\symbol{169}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FAone\symbol{170}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FAone\symbol{171}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FAone\symbol{172}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FAone\symbol{173}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FAone\symbol{174}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FAone\symbol{175}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FAone\symbol{176}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FAone\symbol{177}}}
\expandafter\def\csname faicon@registered\endcsname{{\FAone\symbol{178}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FAone\symbol{179}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FAone\symbol{180}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FAone\symbol{181}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FAone\symbol{182}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FAone\symbol{183}}}
\expandafter\def\csname faicon@safari\endcsname{{\FAone\symbol{184}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FAone\symbol{185}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FAone\symbol{186}}}
\expandafter\def\csname faicon@opera\endcsname{{\FAone\symbol{187}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FAone\symbol{188}}}
\expandafter\def\csname faicon@television\endcsname{{\FAone\symbol{189}}}
\expandafter\def\csname faicon@contao\endcsname{{\FAone\symbol{190}}}
\expandafter\def\csname faicon@500px\endcsname{{\FAone\symbol{191}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FAone\symbol{192}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FAone\symbol{193}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FAone\symbol{194}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FAone\symbol{195}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FAone\symbol{196}}}
\expandafter\def\csname faicon@industry\endcsname{{\FAone\symbol{197}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FAone\symbol{198}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FAone\symbol{199}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FAone\symbol{200}}}
\expandafter\def\csname faicon@map\endcsname{{\FAone\symbol{201}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FAone\symbol{202}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FAone\symbol{203}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FAone\symbol{204}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FAone\symbol{205}}}
\expandafter\def\csname faicon@edge\endcsname{{\FAone\symbol{206}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FAone\symbol{207}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FAone\symbol{208}}}
\expandafter\def\csname faicon@usb\endcsname{{\FAone\symbol{209}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FAone\symbol{210}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FAone\symbol{211}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FAone\symbol{212}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FAone\symbol{213}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FAone\symbol{214}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FAone\symbol{215}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FAone\symbol{216}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FAone\symbol{217}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FAone\symbol{218}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FAone\symbol{219}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FAone\symbol{220}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FAone\symbol{221}}}
\expandafter\def\csname faicon@percent\endcsname{{\FAone\symbol{222}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FAone\symbol{223}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FAone\symbol{224}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FAone\symbol{225}}}
\expandafter\def\csname faicon@envira\endcsname{{\FAone\symbol{226}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FAone\symbol{227}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FAone\symbol{228}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FAone\symbol{229}}}
\expandafter\def\csname faicon@blind\endcsname{{\FAone\symbol{230}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FAone\symbol{231}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FAone\symbol{232}}}
\expandafter\def\csname faicon@adn\endcsname{{\FAone\symbol{233}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FAone\symbol{234}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FAone\symbol{235}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FAone\symbol{236}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FAone\symbol{237}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FAone\symbol{238}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FAone\symbol{239}}}
\expandafter\def\csname faicon@android\endcsname{{\FAone\symbol{240}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FAone\symbol{241}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FAone\symbol{242}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FAone\symbol{243}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FAone\symbol{244}}}
\expandafter\def\csname faicon@apple\endcsname{{\FAone\symbol{245}}}
\expandafter\def\csname faicon@archive\endcsname{{\FAone\symbol{246}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FAone\symbol{247}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FAone\symbol{248}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FAone\symbol{249}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FAone\symbol{250}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FAone\symbol{251}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FAone\symbol{252}}}
\expandafter\def\csname faicon@backward\endcsname{{\FAone\symbol{253}}}
\expandafter\def\csname faicon@ban\endcsname{{\FAone\symbol{254}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FAone\symbol{255}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FAtwo\symbol{0}}}
\expandafter\def\csname faicon@flask\endcsname{{\FAtwo\symbol{1}}}
\expandafter\def\csname faicon@beer\endcsname{{\FAtwo\symbol{2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FAtwo\symbol{3}}}
\expandafter\def\csname faicon@bell\endcsname{{\FAtwo\symbol{4}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FAtwo\symbol{5}}}
\expandafter\def\csname faicon@bold\endcsname{{\FAtwo\symbol{6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FAtwo\symbol{7}}}
\expandafter\def\csname faicon@book\endcsname{{\FAtwo\symbol{8}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FAtwo\symbol{9}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FAtwo\symbol{10}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FAtwo\symbol{11}}}
\expandafter\def\csname faicon@btc\endcsname{{\FAtwo\symbol{12}}}
\expandafter\def\csname faicon@bug\endcsname{{\FAtwo\symbol{13}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FAtwo\symbol{14}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FAtwo\symbol{15}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FAtwo\symbol{16}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FAtwo\symbol{17}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FAtwo\symbol{18}}}
\expandafter\def\csname faicon@camera\endcsname{{\FAtwo\symbol{19}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FAtwo\symbol{20}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FAtwo\symbol{21}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FAtwo\symbol{22}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FAtwo\symbol{23}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FAtwo\symbol{24}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FAtwo\symbol{25}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FAtwo\symbol{26}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FAtwo\symbol{27}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FAtwo\symbol{28}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FAtwo\symbol{29}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FAtwo\symbol{30}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FAtwo\symbol{31}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FAtwo\symbol{32}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FAtwo\symbol{33}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FAtwo\symbol{34}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FAtwo\symbol{35}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FAtwo\symbol{36}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FAtwo\symbol{37}}}
\expandafter\def\csname faicon@circle\endcsname{{\FAtwo\symbol{38}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FAtwo\symbol{39}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FAtwo\symbol{40}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FAtwo\symbol{41}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FAtwo\symbol{42}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FAtwo\symbol{43}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FAtwo\symbol{44}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FAtwo\symbol{45}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FAtwo\symbol{46}}}
\expandafter\def\csname faicon@code\endcsname{{\FAtwo\symbol{47}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FAtwo\symbol{48}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FAtwo\symbol{49}}}
\expandafter\def\csname faicon@cog\endcsname{{\FAtwo\symbol{50}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FAtwo\symbol{51}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FAtwo\symbol{52}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FAtwo\symbol{53}}}
\expandafter\def\csname faicon@columns\endcsname{{\FAtwo\symbol{54}}}
\expandafter\def\csname faicon@comment\endcsname{{\FAtwo\symbol{55}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FAtwo\symbol{56}}}
\expandafter\def\csname faicon@comments\endcsname{{\FAtwo\symbol{57}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FAtwo\symbol{58}}}
\expandafter\def\csname faicon@compass\endcsname{{\FAtwo\symbol{59}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FAtwo\symbol{60}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FAtwo\symbol{61}}}
\expandafter\def\csname faicon@crop\endcsname{{\FAtwo\symbol{62}}}
\expandafter\def\csname faicon@css3\endcsname{{\FAtwo\symbol{63}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FAtwo\symbol{64}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FAtwo\symbol{65}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FAtwo\symbol{66}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FAtwo\symbol{67}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FAtwo\symbol{68}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FAtwo\symbol{69}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FAtwo\symbol{70}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FAtwo\symbol{71}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FAtwo\symbol{72}}}
\expandafter\def\csname faicon@download\endcsname{{\FAtwo\symbol{73}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FAtwo\symbol{74}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FAtwo\symbol{75}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FAtwo\symbol{76}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FAtwo\symbol{77}}}
\expandafter\def\csname faicon@eject\endcsname{{\FAtwo\symbol{78}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FAtwo\symbol{79}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FAtwo\symbol{80}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FAtwo\symbol{81}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FAtwo\symbol{82}}}
\expandafter\def\csname faicon@eur\endcsname{{\FAtwo\symbol{83}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FAtwo\symbol{84}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FAtwo\symbol{85}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FAtwo\symbol{86}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FAtwo\symbol{87}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FAtwo\symbol{88}}}
\expandafter\def\csname faicon@eye\endcsname{{\FAtwo\symbol{89}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FAtwo\symbol{90}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FAtwo\symbol{91}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FAtwo\symbol{92}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FAtwo\symbol{93}}}
\expandafter\def\csname faicon@language\endcsname{{\FAtwo\symbol{94}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FAtwo\symbol{95}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FAtwo\symbol{96}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FAtwo\symbol{97}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FAtwo\symbol{98}}}
\expandafter\def\csname faicon@gg\endcsname{{\FAtwo\symbol{99}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FAtwo\symbol{100}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FAtwo\symbol{101}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FAtwo\symbol{102}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FAtwo\symbol{103}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FAtwo\symbol{104}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FAtwo\symbol{105}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FAtwo\symbol{106}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FAtwo\symbol{107}}}
\expandafter\def\csname faicon@female\endcsname{{\FAtwo\symbol{108}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FAtwo\symbol{109}}}
\expandafter\def\csname faicon@file\endcsname{{\FAtwo\symbol{110}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FAtwo\symbol{111}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FAtwo\symbol{112}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FAtwo\symbol{113}}}
\expandafter\def\csname faicon@film\endcsname{{\FAtwo\symbol{114}}}
\expandafter\def\csname faicon@filter\endcsname{{\FAtwo\symbol{115}}}
\expandafter\def\csname faicon@fire\endcsname{{\FAtwo\symbol{116}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FAtwo\symbol{117}}}
\expandafter\def\csname faicon@flag\endcsname{{\FAtwo\symbol{118}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FAtwo\symbol{119}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FAtwo\symbol{120}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FAtwo\symbol{121}}}
\expandafter\def\csname faicon@folder\endcsname{{\FAtwo\symbol{122}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FAtwo\symbol{123}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FAtwo\symbol{124}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FAtwo\symbol{125}}}
\expandafter\def\csname faicon@font\endcsname{{\FAtwo\symbol{126}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FAtwo\symbol{127}}}
\expandafter\def\csname faicon@forward\endcsname{{\FAtwo\symbol{128}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FAtwo\symbol{129}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FAtwo\symbol{130}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FAtwo\symbol{131}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FAtwo\symbol{132}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FAtwo\symbol{133}}}
\expandafter\def\csname faicon@gift\endcsname{{\FAtwo\symbol{134}}}
\expandafter\def\csname faicon@github\endcsname{{\FAtwo\symbol{135}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FAtwo\symbol{136}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FAtwo\symbol{137}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FAtwo\symbol{138}}}
\expandafter\def\csname faicon@glass\endcsname{{\FAtwo\symbol{139}}}
\expandafter\def\csname faicon@globe\endcsname{{\FAtwo\symbol{140}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FAtwo\symbol{141}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FAtwo\symbol{142}}}
\expandafter\def\csname faicon@users\endcsname{{\FAtwo\symbol{143}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FAtwo\symbol{144}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FAtwo\symbol{145}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FAtwo\symbol{146}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FAtwo\symbol{147}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FAtwo\symbol{148}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FAtwo\symbol{149}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FAtwo\symbol{150}}}
\expandafter\def\csname faicon@heart\endcsname{{\FAtwo\symbol{151}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FAtwo\symbol{152}}}
\expandafter\def\csname faicon@home\endcsname{{\FAtwo\symbol{153}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FAtwo\symbol{154}}}
\expandafter\def\csname faicon@html5\endcsname{{\FAtwo\symbol{155}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FAtwo\symbol{156}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FAtwo\symbol{157}}}
\expandafter\def\csname faicon@indent\endcsname{{\FAtwo\symbol{158}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FAtwo\symbol{159}}}
\expandafter\def\csname faicon@inr\endcsname{{\FAtwo\symbol{160}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FAtwo\symbol{161}}}
\expandafter\def\csname faicon@italic\endcsname{{\FAtwo\symbol{162}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FAtwo\symbol{163}}}
\expandafter\def\csname faicon@key\endcsname{{\FAtwo\symbol{164}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FAtwo\symbol{165}}}
\expandafter\def\csname faicon@krw\endcsname{{\FAtwo\symbol{166}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FAtwo\symbol{167}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FAtwo\symbol{168}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FAtwo\symbol{169}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FAtwo\symbol{170}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FAtwo\symbol{171}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FAtwo\symbol{172}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FAtwo\symbol{173}}}
\expandafter\def\csname faicon@link\endcsname{{\FAtwo\symbol{174}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FAtwo\symbol{175}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FAtwo\symbol{176}}}
\expandafter\def\csname faicon@linux\endcsname{{\FAtwo\symbol{177}}}
\expandafter\def\csname faicon@list\endcsname{{\FAtwo\symbol{178}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FAtwo\symbol{179}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FAtwo\symbol{180}}}
\expandafter\def\csname faicon@lock\endcsname{{\FAtwo\symbol{181}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FAtwo\symbol{182}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FAtwo\symbol{183}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FAtwo\symbol{184}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FAtwo\symbol{185}}}
\expandafter\def\csname faicon@magic\endcsname{{\FAtwo\symbol{186}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FAtwo\symbol{187}}}
\expandafter\def\csname faicon@male\endcsname{{\FAtwo\symbol{188}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FAtwo\symbol{189}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FAtwo\symbol{190}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FAtwo\symbol{191}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FAtwo\symbol{192}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FAtwo\symbol{193}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FAtwo\symbol{194}}}
\expandafter\def\csname faicon@minus\endcsname{{\FAtwo\symbol{195}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FAtwo\symbol{196}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FAtwo\symbol{197}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FAtwo\symbol{198}}}
\expandafter\def\csname faicon@money\endcsname{{\FAtwo\symbol{199}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FAtwo\symbol{200}}}
\expandafter\def\csname faicon@music\endcsname{{\FAtwo\symbol{201}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FAtwo\symbol{202}}}
\expandafter\def\csname faicon@check\endcsname{{\FAtwo\symbol{203}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FAtwo\symbol{204}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FAtwo\symbol{205}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FAtwo\symbol{206}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FAtwo\symbol{207}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FAtwo\symbol{208}}}
\expandafter\def\csname faicon@pause\endcsname{{\FAtwo\symbol{209}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FAtwo\symbol{210}}}
\expandafter\def\csname faicon@phone\endcsname{{\FAtwo\symbol{211}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FAtwo\symbol{212}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FAtwo\symbol{213}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FAtwo\symbol{214}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FAtwo\symbol{215}}}
\expandafter\def\csname faicon@plane\endcsname{{\FAtwo\symbol{216}}}
\expandafter\def\csname faicon@play\endcsname{{\FAtwo\symbol{217}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FAtwo\symbol{218}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FAtwo\symbol{219}}}
\expandafter\def\csname faicon@plus\endcsname{{\FAtwo\symbol{220}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FAtwo\symbol{221}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FAtwo\symbol{222}}}
\expandafter\def\csname faicon@print\endcsname{{\FAtwo\symbol{223}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FAtwo\symbol{224}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FAtwo\symbol{225}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FAtwo\symbol{226}}}
\expandafter\def\csname faicon@question\endcsname{{\FAtwo\symbol{227}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FAtwo\symbol{228}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FAtwo\symbol{229}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FAtwo\symbol{230}}}
\expandafter\def\csname faicon@random\endcsname{{\FAtwo\symbol{231}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FAtwo\symbol{232}}}
\expandafter\def\csname faicon@times\endcsname{{\FAtwo\symbol{233}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FAtwo\symbol{234}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FAtwo\symbol{235}}}
\expandafter\def\csname faicon@renren\endcsname{{\FAtwo\symbol{236}}}
\expandafter\def\csname faicon@bars\endcsname{{\FAtwo\symbol{237}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FAtwo\symbol{238}}}
\expandafter\def\csname faicon@reply\endcsname{{\FAtwo\symbol{239}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FAtwo\symbol{240}}}
\expandafter\def\csname faicon@expand\endcsname{{\FAtwo\symbol{241}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FAtwo\symbol{242}}}
\expandafter\def\csname faicon@compress\endcsname{{\FAtwo\symbol{243}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FAtwo\symbol{244}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FAtwo\symbol{245}}}
\expandafter\def\csname faicon@road\endcsname{{\FAtwo\symbol{246}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FAtwo\symbol{247}}}
\expandafter\def\csname faicon@rss\endcsname{{\FAtwo\symbol{248}}}
\expandafter\def\csname faicon@rub\endcsname{{\FAtwo\symbol{249}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FAtwo\symbol{250}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FAtwo\symbol{251}}}
\expandafter\def\csname faicon@search\endcsname{{\FAtwo\symbol{252}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FAtwo\symbol{253}}}
\expandafter\def\csname faicon@share\endcsname{{\FAtwo\symbol{254}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FAtwo\symbol{255}}}
\expandafter\def\csname faicon@shield\endcsname{{\FAthree\symbol{0}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FAthree\symbol{1}}}
\expandafter\def\csname faicon@square\endcsname{{\FAthree\symbol{2}}}
\expandafter\def\csname faicon@signal\endcsname{{\FAthree\symbol{3}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FAthree\symbol{4}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FAthree\symbol{5}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FAthree\symbol{6}}}
\expandafter\def\csname faicon@skype\endcsname{{\FAthree\symbol{7}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FAthree\symbol{8}}}
\expandafter\def\csname faicon@sort\endcsname{{\FAthree\symbol{9}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FAthree\symbol{10}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FAthree\symbol{11}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FAthree\symbol{12}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FAthree\symbol{13}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FAthree\symbol{14}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FAthree\symbol{15}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FAthree\symbol{16}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FAthree\symbol{17}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FAthree\symbol{18}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FAthree\symbol{19}}}
\expandafter\def\csname faicon@star\endcsname{{\FAthree\symbol{20}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FAthree\symbol{21}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FAthree\symbol{22}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FAthree\symbol{23}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FAthree\symbol{24}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FAthree\symbol{25}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FAthree\symbol{26}}}
\expandafter\def\csname faicon@stop\endcsname{{\FAthree\symbol{27}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FAthree\symbol{28}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FAthree\symbol{29}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FAthree\symbol{30}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FAthree\symbol{31}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FAthree\symbol{32}}}
\expandafter\def\csname faicon@table\endcsname{{\FAthree\symbol{33}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FAthree\symbol{34}}}
\expandafter\def\csname faicon@tag\endcsname{{\FAthree\symbol{35}}}
\expandafter\def\csname faicon@tags\endcsname{{\FAthree\symbol{36}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FAthree\symbol{37}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FAthree\symbol{38}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FAthree\symbol{39}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FAthree\symbol{40}}}
\expandafter\def\csname faicon@th\endcsname{{\FAthree\symbol{41}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FAthree\symbol{42}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FAthree\symbol{43}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FAthree\symbol{44}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FAthree\symbol{45}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FAthree\symbol{46}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FAthree\symbol{47}}}
\expandafter\def\csname faicon@tint\endcsname{{\FAthree\symbol{48}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FAthree\symbol{49}}}
\expandafter\def\csname faicon@trello\endcsname{{\FAthree\symbol{50}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FAthree\symbol{51}}}
\expandafter\def\csname faicon@truck\endcsname{{\FAthree\symbol{52}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FAthree\symbol{53}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FAthree\symbol{54}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FAthree\symbol{55}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FAthree\symbol{56}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FAthree\symbol{57}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FAthree\symbol{58}}}
\expandafter\def\csname faicon@underline\endcsname{{\FAthree\symbol{59}}}
\expandafter\def\csname faicon@undo\endcsname{{\FAthree\symbol{60}}}
\expandafter\def\csname faicon@google\endcsname{{\FAthree\symbol{61}}}
\expandafter\def\csname faicon@paw\endcsname{{\FAthree\symbol{62}}}
\expandafter\def\csname faicon@database\endcsname{{\FAthree\symbol{63}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FAthree\symbol{64}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FAthree\symbol{65}}}
\expandafter\def\csname faicon@empire\endcsname{{\FAthree\symbol{66}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FAthree\symbol{67}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FAthree\symbol{68}}}
\expandafter\def\csname faicon@qq\endcsname{{\FAthree\symbol{69}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FAthree\symbol{70}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FAthree\symbol{71}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FAthree\symbol{72}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FAthree\symbol{73}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FAthree\symbol{74}}}
\expandafter\def\csname faicon@modx\endcsname{{\FAthree\symbol{75}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FAthree\symbol{76}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FAthree\symbol{77}}}
\expandafter\def\csname faicon@braille\endcsname{{\FAthree\symbol{78}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FAthree\symbol{79}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FAthree\symbol{80}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FAthree\symbol{81}}}
\expandafter\def\csname faicon@glide\endcsname{{\FAthree\symbol{82}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FAthree\symbol{83}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FAthree\symbol{84}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FAthree\symbol{85}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FAthree\symbol{86}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FAthree\symbol{87}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FAthree\symbol{88}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FAthree\symbol{89}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FAthree\symbol{90}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FAthree\symbol{91}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FAthree\symbol{92}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FAthree\symbol{93}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FAthree\symbol{94}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FAthree\symbol{95}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FAthree\symbol{96}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FAthree\symbol{97}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FAthree\symbol{98}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FAthree\symbol{99}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FAthree\symbol{100}}}
\expandafter\def\csname faicon@upload\endcsname{{\FAthree\symbol{101}}}
\expandafter\def\csname faicon@usd\endcsname{{\FAthree\symbol{102}}}
\expandafter\def\csname faicon@user\endcsname{{\FAthree\symbol{103}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FAthree\symbol{104}}}
\expandafter\def\csname faicon@venus\endcsname{{\FAthree\symbol{105}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FAthree\symbol{106}}}
\expandafter\def\csname faicon@vk\endcsname{{\FAthree\symbol{107}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FAthree\symbol{108}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FAthree\symbol{109}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FAthree\symbol{110}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FAthree\symbol{111}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FAthree\symbol{112}}}
\expandafter\def\csname faicon@windows\endcsname{{\FAthree\symbol{113}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FAthree\symbol{114}}}
\expandafter\def\csname faicon@xing\endcsname{{\FAthree\symbol{115}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FAthree\symbol{116}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FAthree\symbol{117}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FAthree\symbol{118}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FAthree\symbol{119}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FAthree\symbol{120}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FAthree\symbol{121}}}

%% end of file `fontawesomesymbols-pdftex.tex'.


==> fontawesomesymbols-xeluatex.tex <==
\expandafter\def\csname faicon@glass\endcsname{{\FA\symbol{"F000}}}
\expandafter\def\csname faicon@music\endcsname{{\FA\symbol{"F001}}}
\expandafter\def\csname faicon@search\endcsname{{\FA\symbol{"F002}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FA\symbol{"F003}}}
\expandafter\def\csname faicon@heart\endcsname{{\FA\symbol{"F004}}}
\expandafter\def\csname faicon@star\endcsname{{\FA\symbol{"F005}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FA\symbol{"F006}}}
\expandafter\def\csname faicon@user\endcsname{{\FA\symbol{"F007}}}
\expandafter\def\csname faicon@film\endcsname{{\FA\symbol{"F008}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FA\symbol{"F009}}}
\expandafter\def\csname faicon@th\endcsname{{\FA\symbol{"F00A}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FA\symbol{"F00B}}}
\expandafter\def\csname faicon@check\endcsname{{\FA\symbol{"F00C}}}
\expandafter\def\csname faicon@times\endcsname{{\FA\symbol{"F00D}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FA\symbol{"F00E}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FA\symbol{"F010}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FA\symbol{"F011}}}
\expandafter\def\csname faicon@signal\endcsname{{\FA\symbol{"F012}}}
\expandafter\def\csname faicon@cog\endcsname{{\FA\symbol{"F013}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FA\symbol{"F014}}}
\expandafter\def\csname faicon@home\endcsname{{\FA\symbol{"F015}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FA\symbol{"F016}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FA\symbol{"F017}}}
\expandafter\def\csname faicon@road\endcsname{{\FA\symbol{"F018}}}
\expandafter\def\csname faicon@download\endcsname{{\FA\symbol{"F019}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FA\symbol{"F01A}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FA\symbol{"F01B}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FA\symbol{"F01C}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FA\symbol{"F01D}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FA\symbol{"F01E}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FA\symbol{"F021}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FA\symbol{"F022}}}
\expandafter\def\csname faicon@lock\endcsname{{\FA\symbol{"F023}}}
\expandafter\def\csname faicon@flag\endcsname{{\FA\symbol{"F024}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FA\symbol{"F025}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FA\symbol{"F026}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FA\symbol{"F027}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FA\symbol{"F028}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FA\symbol{"F029}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FA\symbol{"F02A}}}
\expandafter\def\csname faicon@tag\endcsname{{\FA\symbol{"F02B}}}
\expandafter\def\csname faicon@tags\endcsname{{\FA\symbol{"F02C}}}
\expandafter\def\csname faicon@book\endcsname{{\FA\symbol{"F02D}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FA\symbol{"F02E}}}
\expandafter\def\csname faicon@print\endcsname{{\FA\symbol{"F02F}}}
\expandafter\def\csname faicon@camera\endcsname{{\FA\symbol{"F030}}}
\expandafter\def\csname faicon@font\endcsname{{\FA\symbol{"F031}}}
\expandafter\def\csname faicon@bold\endcsname{{\FA\symbol{"F032}}}
\expandafter\def\csname faicon@italic\endcsname{{\FA\symbol{"F033}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FA\symbol{"F034}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FA\symbol{"F035}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FA\symbol{"F036}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FA\symbol{"F037}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FA\symbol{"F038}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FA\symbol{"F039}}}
\expandafter\def\csname faicon@list\endcsname{{\FA\symbol{"F03A}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FA\symbol{"F03B}}}
\expandafter\def\csname faicon@indent\endcsname{{\FA\symbol{"F03C}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FA\symbol{"F03D}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FA\symbol{"F03E}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FA\symbol{"F040}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FA\symbol{"F041}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FA\symbol{"F042}}}
\expandafter\def\csname faicon@tint\endcsname{{\FA\symbol{"F043}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FA\symbol{"F044}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FA\symbol{"F045}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FA\symbol{"F046}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FA\symbol{"F047}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FA\symbol{"F048}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FA\symbol{"F049}}}
\expandafter\def\csname faicon@backward\endcsname{{\FA\symbol{"F04A}}}
\expandafter\def\csname faicon@play\endcsname{{\FA\symbol{"F04B}}}
\expandafter\def\csname faicon@pause\endcsname{{\FA\symbol{"F04C}}}
\expandafter\def\csname faicon@stop\endcsname{{\FA\symbol{"F04D}}}
\expandafter\def\csname faicon@forward\endcsname{{\FA\symbol{"F04E}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FA\symbol{"F050}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FA\symbol{"F051}}}
\expandafter\def\csname faicon@eject\endcsname{{\FA\symbol{"F052}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FA\symbol{"F053}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FA\symbol{"F054}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FA\symbol{"F055}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FA\symbol{"F056}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FA\symbol{"F057}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FA\symbol{"F058}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FA\symbol{"F059}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FA\symbol{"F05A}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FA\symbol{"F05B}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FA\symbol{"F05C}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FA\symbol{"F05D}}}
\expandafter\def\csname faicon@ban\endcsname{{\FA\symbol{"F05E}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FA\symbol{"F060}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FA\symbol{"F061}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FA\symbol{"F062}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FA\symbol{"F063}}}
\expandafter\def\csname faicon@share\endcsname{{\FA\symbol{"F064}}}
\expandafter\def\csname faicon@expand\endcsname{{\FA\symbol{"F065}}}
\expandafter\def\csname faicon@compress\endcsname{{\FA\symbol{"F066}}}
\expandafter\def\csname faicon@plus\endcsname{{\FA\symbol{"F067}}}
\expandafter\def\csname faicon@minus\endcsname{{\FA\symbol{"F068}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FA\symbol{"F069}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FA\symbol{"F06A}}}
\expandafter\def\csname faicon@gift\endcsname{{\FA\symbol{"F06B}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FA\symbol{"F06C}}}
\expandafter\def\csname faicon@fire\endcsname{{\FA\symbol{"F06D}}}
\expandafter\def\csname faicon@eye\endcsname{{\FA\symbol{"F06E}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FA\symbol{"F070}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FA\symbol{"F071}}}
\expandafter\def\csname faicon@plane\endcsname{{\FA\symbol{"F072}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FA\symbol{"F073}}}
\expandafter\def\csname faicon@random\endcsname{{\FA\symbol{"F074}}}
\expandafter\def\csname faicon@comment\endcsname{{\FA\symbol{"F075}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FA\symbol{"F076}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FA\symbol{"F077}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FA\symbol{"F078}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FA\symbol{"F079}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FA\symbol{"F07A}}}
\expandafter\def\csname faicon@folder\endcsname{{\FA\symbol{"F07B}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FA\symbol{"F07C}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FA\symbol{"F07D}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FA\symbol{"F07E}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FA\symbol{"F080}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FA\symbol{"F081}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FA\symbol{"F082}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FA\symbol{"F083}}}
\expandafter\def\csname faicon@key\endcsname{{\FA\symbol{"F084}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FA\symbol{"F085}}}
\expandafter\def\csname faicon@comments\endcsname{{\FA\symbol{"F086}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FA\symbol{"F087}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FA\symbol{"F088}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FA\symbol{"F089}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FA\symbol{"F08A}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FA\symbol{"F08B}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FA\symbol{"F08C}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FA\symbol{"F08D}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FA\symbol{"F08E}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FA\symbol{"F090}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FA\symbol{"F091}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FA\symbol{"F092}}}
\expandafter\def\csname faicon@upload\endcsname{{\FA\symbol{"F093}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FA\symbol{"F094}}}
\expandafter\def\csname faicon@phone\endcsname{{\FA\symbol{"F095}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FA\symbol{"F096}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FA\symbol{"F097}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FA\symbol{"F098}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FA\symbol{"F099}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FA\symbol{"F09A}}}
\expandafter\def\csname faicon@github\endcsname{{\FA\symbol{"F09B}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FA\symbol{"F09C}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FA\symbol{"F09D}}}
\expandafter\def\csname faicon@rss\endcsname{{\FA\symbol{"F09E}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FA\symbol{"F0A0}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FA\symbol{"F0A1}}}
\expandafter\def\csname faicon@bell\endcsname{{\FA\symbol{"F0F3}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FA\symbol{"F0A3}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FA\symbol{"F0A4}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FA\symbol{"F0A5}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FA\symbol{"F0A6}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FA\symbol{"F0A7}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FA\symbol{"F0A8}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FA\symbol{"F0A9}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FA\symbol{"F0AA}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FA\symbol{"F0AB}}}
\expandafter\def\csname faicon@globe\endcsname{{\FA\symbol{"F0AC}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FA\symbol{"F0AD}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FA\symbol{"F0AE}}}
\expandafter\def\csname faicon@filter\endcsname{{\FA\symbol{"F0B0}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FA\symbol{"F0B1}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FA\symbol{"F0B2}}}
\expandafter\def\csname faicon@users\endcsname{{\FA\symbol{"F0C0}}}
\expandafter\def\csname faicon@link\endcsname{{\FA\symbol{"F0C1}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FA\symbol{"F0C2}}}
\expandafter\def\csname faicon@flask\endcsname{{\FA\symbol{"F0C3}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FA\symbol{"F0C4}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FA\symbol{"F0C5}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FA\symbol{"F0C6}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FA\symbol{"F0C7}}}
\expandafter\def\csname faicon@square\endcsname{{\FA\symbol{"F0C8}}}
\expandafter\def\csname faicon@bars\endcsname{{\FA\symbol{"F0C9}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FA\symbol{"F0CA}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FA\symbol{"F0CB}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FA\symbol{"F0CC}}}
\expandafter\def\csname faicon@underline\endcsname{{\FA\symbol{"F0CD}}}
\expandafter\def\csname faicon@table\endcsname{{\FA\symbol{"F0CE}}}
\expandafter\def\csname faicon@magic\endcsname{{\FA\symbol{"F0D0}}}
\expandafter\def\csname faicon@truck\endcsname{{\FA\symbol{"F0D1}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FA\symbol{"F0D2}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FA\symbol{"F0D3}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FA\symbol{"F0D4}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FA\symbol{"F0D5}}}
\expandafter\def\csname faicon@money\endcsname{{\FA\symbol{"F0D6}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FA\symbol{"F0D7}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FA\symbol{"F0D8}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FA\symbol{"F0D9}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FA\symbol{"F0DA}}}
\expandafter\def\csname faicon@columns\endcsname{{\FA\symbol{"F0DB}}}
\expandafter\def\csname faicon@sort\endcsname{{\FA\symbol{"F0DC}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FA\symbol{"F0DD}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FA\symbol{"F0DE}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FA\symbol{"F0E0}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FA\symbol{"F0E1}}}
\expandafter\def\csname faicon@undo\endcsname{{\FA\symbol{"F0E2}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FA\symbol{"F0E3}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FA\symbol{"F0E4}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FA\symbol{"F0E5}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FA\symbol{"F0E6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FA\symbol{"F0E7}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FA\symbol{"F0E8}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FA\symbol{"F0E9}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FA\symbol{"F0EA}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FA\symbol{"F0EB}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FA\symbol{"F0EC}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FA\symbol{"F0ED}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FA\symbol{"F0EE}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FA\symbol{"F0F0}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FA\symbol{"F0F1}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FA\symbol{"F0F2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FA\symbol{"F0A2}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FA\symbol{"F0F4}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FA\symbol{"F0F5}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FA\symbol{"F0F6}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FA\symbol{"F0F7}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FA\symbol{"F0F8}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FA\symbol{"F0F9}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FA\symbol{"F0FA}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FA\symbol{"F0FB}}}
\expandafter\def\csname faicon@beer\endcsname{{\FA\symbol{"F0FC}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FA\symbol{"F0FD}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FA\symbol{"F0FE}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FA\symbol{"F100}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FA\symbol{"F101}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FA\symbol{"F102}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FA\symbol{"F103}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FA\symbol{"F104}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FA\symbol{"F105}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FA\symbol{"F106}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FA\symbol{"F107}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FA\symbol{"F108}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FA\symbol{"F109}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FA\symbol{"F10A}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FA\symbol{"F10B}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FA\symbol{"F10C}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FA\symbol{"F10D}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FA\symbol{"F10E}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FA\symbol{"F110}}}
\expandafter\def\csname faicon@circle\endcsname{{\FA\symbol{"F111}}}
\expandafter\def\csname faicon@reply\endcsname{{\FA\symbol{"F112}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FA\symbol{"F113}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FA\symbol{"F114}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FA\symbol{"F115}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FA\symbol{"F118}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FA\symbol{"F119}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FA\symbol{"F11A}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FA\symbol{"F11B}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FA\symbol{"F11C}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FA\symbol{"F11D}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FA\symbol{"F11E}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FA\symbol{"F120}}}
\expandafter\def\csname faicon@code\endcsname{{\FA\symbol{"F121}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FA\symbol{"F122}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FA\symbol{"F123}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FA\symbol{"F124}}}
\expandafter\def\csname faicon@crop\endcsname{{\FA\symbol{"F125}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FA\symbol{"F126}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FA\symbol{"F127}}}
\expandafter\def\csname faicon@question\endcsname{{\FA\symbol{"F128}}}
\expandafter\def\csname faicon@info\endcsname{{\FA\symbol{"F129}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FA\symbol{"F12A}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FA\symbol{"F12B}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FA\symbol{"F12C}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FA\symbol{"F12D}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FA\symbol{"F12E}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FA\symbol{"F130}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FA\symbol{"F131}}}
\expandafter\def\csname faicon@shield\endcsname{{\FA\symbol{"F132}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FA\symbol{"F133}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FA\symbol{"F134}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FA\symbol{"F135}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FA\symbol{"F136}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FA\symbol{"F137}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FA\symbol{"F138}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FA\symbol{"F139}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FA\symbol{"F13A}}}
\expandafter\def\csname faicon@html5\endcsname{{\FA\symbol{"F13B}}}
\expandafter\def\csname faicon@css3\endcsname{{\FA\symbol{"F13C}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FA\symbol{"F13D}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FA\symbol{"F13E}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FA\symbol{"F140}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FA\symbol{"F141}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FA\symbol{"F142}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FA\symbol{"F143}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FA\symbol{"F144}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FA\symbol{"F145}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FA\symbol{"F146}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FA\symbol{"F147}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FA\symbol{"F148}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FA\symbol{"F149}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FA\symbol{"F14A}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FA\symbol{"F14B}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FA\symbol{"F14C}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FA\symbol{"F14D}}}
\expandafter\def\csname faicon@compass\endcsname{{\FA\symbol{"F14E}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FA\symbol{"F150}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FA\symbol{"F151}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FA\symbol{"F152}}}
\expandafter\def\csname faicon@eur\endcsname{{\FA\symbol{"F153}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FA\symbol{"F154}}}
\expandafter\def\csname faicon@usd\endcsname{{\FA\symbol{"F155}}}
\expandafter\def\csname faicon@inr\endcsname{{\FA\symbol{"F156}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FA\symbol{"F157}}}
\expandafter\def\csname faicon@rub\endcsname{{\FA\symbol{"F158}}}
\expandafter\def\csname faicon@krw\endcsname{{\FA\symbol{"F159}}}
\expandafter\def\csname faicon@btc\endcsname{{\FA\symbol{"F15A}}}
\expandafter\def\csname faicon@file\endcsname{{\FA\symbol{"F15B}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FA\symbol{"F15C}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FA\symbol{"F15D}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FA\symbol{"F15E}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FA\symbol{"F160}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FA\symbol{"F161}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FA\symbol{"F162}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FA\symbol{"F163}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FA\symbol{"F164}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FA\symbol{"F165}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FA\symbol{"F166}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FA\symbol{"F167}}}
\expandafter\def\csname faicon@xing\endcsname{{\FA\symbol{"F168}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FA\symbol{"F169}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FA\symbol{"F16A}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FA\symbol{"F16B}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FA\symbol{"F16C}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FA\symbol{"F16D}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FA\symbol{"F16E}}}
\expandafter\def\csname faicon@adn\endcsname{{\FA\symbol{"F170}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FA\symbol{"F171}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FA\symbol{"F172}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FA\symbol{"F173}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FA\symbol{"F174}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FA\symbol{"F175}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FA\symbol{"F176}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FA\symbol{"F177}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FA\symbol{"F178}}}
\expandafter\def\csname faicon@apple\endcsname{{\FA\symbol{"F179}}}
\expandafter\def\csname faicon@windows\endcsname{{\FA\symbol{"F17A}}}
\expandafter\def\csname faicon@android\endcsname{{\FA\symbol{"F17B}}}
\expandafter\def\csname faicon@linux\endcsname{{\FA\symbol{"F17C}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FA\symbol{"F17D}}}
\expandafter\def\csname faicon@skype\endcsname{{\FA\symbol{"F17E}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FA\symbol{"F180}}}
\expandafter\def\csname faicon@trello\endcsname{{\FA\symbol{"F181}}}
\expandafter\def\csname faicon@female\endcsname{{\FA\symbol{"F182}}}
\expandafter\def\csname faicon@male\endcsname{{\FA\symbol{"F183}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FA\symbol{"F184}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FA\symbol{"F185}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FA\symbol{"F186}}}
\expandafter\def\csname faicon@archive\endcsname{{\FA\symbol{"F187}}}
\expandafter\def\csname faicon@bug\endcsname{{\FA\symbol{"F188}}}
\expandafter\def\csname faicon@vk\endcsname{{\FA\symbol{"F189}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FA\symbol{"F18A}}}
\expandafter\def\csname faicon@renren\endcsname{{\FA\symbol{"F18B}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FA\symbol{"F18C}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FA\symbol{"F18D}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FA\symbol{"F18E}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FA\symbol{"F190}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FA\symbol{"F191}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FA\symbol{"F192}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FA\symbol{"F193}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FA\symbol{"F194}}}
\expandafter\def\csname faicon@try\endcsname{{\FA\symbol{"F195}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FA\symbol{"F196}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FA\symbol{"F197}}}
\expandafter\def\csname faicon@slack\endcsname{{\FA\symbol{"F198}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FA\symbol{"F199}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FA\symbol{"F19A}}}
\expandafter\def\csname faicon@openid\endcsname{{\FA\symbol{"F19B}}}
\expandafter\def\csname faicon@university\endcsname{{\FA\symbol{"F19C}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FA\symbol{"F19D}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FA\symbol{"F19E}}}
\expandafter\def\csname faicon@google\endcsname{{\FA\symbol{"F1A0}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FA\symbol{"F1A1}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FA\symbol{"F1A2}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FA\symbol{"F1A3}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FA\symbol{"F1A4}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FA\symbol{"F1A5}}}
\expandafter\def\csname faicon@digg\endcsname{{\FA\symbol{"F1A6}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FA\symbol{"F1A7}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FA\symbol{"F1A8}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FA\symbol{"F1A9}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FA\symbol{"F1AA}}}
\expandafter\def\csname faicon@language\endcsname{{\FA\symbol{"F1AB}}}
\expandafter\def\csname faicon@fax\endcsname{{\FA\symbol{"F1AC}}}
\expandafter\def\csname faicon@building\endcsname{{\FA\symbol{"F1AD}}}
\expandafter\def\csname faicon@child\endcsname{{\FA\symbol{"F1AE}}}
\expandafter\def\csname faicon@paw\endcsname{{\FA\symbol{"F1B0}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FA\symbol{"F1B1}}}
\expandafter\def\csname faicon@cube\endcsname{{\FA\symbol{"F1B2}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FA\symbol{"F1B3}}}
\expandafter\def\csname faicon@behance\endcsname{{\FA\symbol{"F1B4}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FA\symbol{"F1B5}}}
\expandafter\def\csname faicon@steam\endcsname{{\FA\symbol{"F1B6}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FA\symbol{"F1B7}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FA\symbol{"F1B8}}}
\expandafter\def\csname faicon@car\endcsname{{\FA\symbol{"F1B9}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FA\symbol{"F1BA}}}
\expandafter\def\csname faicon@tree\endcsname{{\FA\symbol{"F1BB}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FA\symbol{"F1BC}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FA\symbol{"F1BD}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FA\symbol{"F1BE}}}
\expandafter\def\csname faicon@database\endcsname{{\FA\symbol{"F1C0}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FA\symbol{"F1C1}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FA\symbol{"F1C2}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FA\symbol{"F1C3}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FA\symbol{"F1C4}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FA\symbol{"F1C5}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FA\symbol{"F1C6}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FA\symbol{"F1C7}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FA\symbol{"F1C8}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FA\symbol{"F1C9}}}
\expandafter\def\csname faicon@vine\endcsname{{\FA\symbol{"F1CA}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FA\symbol{"F1CB}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FA\symbol{"F1CC}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FA\symbol{"F1CD}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FA\symbol{"F1CE}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FA\symbol{"F1D0}}}
\expandafter\def\csname faicon@empire\endcsname{{\FA\symbol{"F1D1}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FA\symbol{"F1D2}}}
\expandafter\def\csname faicon@git\endcsname{{\FA\symbol{"F1D3}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FA\symbol{"F1D4}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FA\symbol{"F1D5}}}
\expandafter\def\csname faicon@qq\endcsname{{\FA\symbol{"F1D6}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FA\symbol{"F1D7}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FA\symbol{"F1D8}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FA\symbol{"F1D9}}}
\expandafter\def\csname faicon@history\endcsname{{\FA\symbol{"F1DA}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FA\symbol{"F1DB}}}
\expandafter\def\csname faicon@header\endcsname{{\FA\symbol{"F1DC}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FA\symbol{"F1DD}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FA\symbol{"F1DE}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FA\symbol{"F1E0}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FA\symbol{"F1E1}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FA\symbol{"F1E2}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FA\symbol{"F1E3}}}
\expandafter\def\csname faicon@tty\endcsname{{\FA\symbol{"F1E4}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FA\symbol{"F1E5}}}
\expandafter\def\csname faicon@plug\endcsname{{\FA\symbol{"F1E6}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FA\symbol{"F1E7}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FA\symbol{"F1E8}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FA\symbol{"F1E9}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FA\symbol{"F1EA}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FA\symbol{"F1EB}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FA\symbol{"F1EC}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FA\symbol{"F1ED}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FA\symbol{"F1EE}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FA\symbol{"F1F0}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FA\symbol{"F1F1}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FA\symbol{"F1F2}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FA\symbol{"F1F3}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FA\symbol{"F1F4}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FA\symbol{"F1F5}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FA\symbol{"F1F6}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FA\symbol{"F1F7}}}
\expandafter\def\csname faicon@trash\endcsname{{\FA\symbol{"F1F8}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FA\symbol{"F1F9}}}
\expandafter\def\csname faicon@at\endcsname{{\FA\symbol{"F1FA}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FA\symbol{"F1FB}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FA\symbol{"F1FC}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FA\symbol{"F1FD}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FA\symbol{"F1FE}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FA\symbol{"F200}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FA\symbol{"F201}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FA\symbol{"F202}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FA\symbol{"F203}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FA\symbol{"F204}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FA\symbol{"F205}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FA\symbol{"F206}}}
\expandafter\def\csname faicon@bus\endcsname{{\FA\symbol{"F207}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FA\symbol{"F208}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FA\symbol{"F209}}}
\expandafter\def\csname faicon@cc\endcsname{{\FA\symbol{"F20A}}}
\expandafter\def\csname faicon@ils\endcsname{{\FA\symbol{"F20B}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FA\symbol{"F20C}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FA\symbol{"F20D}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FA\symbol{"F20E}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FA\symbol{"F210}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FA\symbol{"F211}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FA\symbol{"F212}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FA\symbol{"F213}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FA\symbol{"F214}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FA\symbol{"F215}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FA\symbol{"F216}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FA\symbol{"F217}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FA\symbol{"F218}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FA\symbol{"F219}}}
\expandafter\def\csname faicon@ship\endcsname{{\FA\symbol{"F21A}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FA\symbol{"F21B}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FA\symbol{"F21C}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FA\symbol{"F21D}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FA\symbol{"F21E}}}
\expandafter\def\csname faicon@venus\endcsname{{\FA\symbol{"F221}}}
\expandafter\def\csname faicon@mars\endcsname{{\FA\symbol{"F222}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FA\symbol{"F223}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FA\symbol{"F224}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FA\symbol{"F225}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FA\symbol{"F226}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FA\symbol{"F227}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FA\symbol{"F228}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FA\symbol{"F229}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FA\symbol{"F22A}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FA\symbol{"F22B}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FA\symbol{"F22C}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FA\symbol{"F22D}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FA\symbol{"F230}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FA\symbol{"F231}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FA\symbol{"F232}}}
\expandafter\def\csname faicon@server\endcsname{{\FA\symbol{"F233}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FA\symbol{"F234}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FA\symbol{"F235}}}
\expandafter\def\csname faicon@bed\endcsname{{\FA\symbol{"F236}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FA\symbol{"F237}}}
\expandafter\def\csname faicon@train\endcsname{{\FA\symbol{"F238}}}
\expandafter\def\csname faicon@subway\endcsname{{\FA\symbol{"F239}}}
\expandafter\def\csname faicon@medium\endcsname{{\FA\symbol{"F23A}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FA\symbol{"F23B}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FA\symbol{"F23C}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FA\symbol{"F23D}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FA\symbol{"F23E}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FA\symbol{"F240}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FA\symbol{"F241}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FA\symbol{"F242}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FA\symbol{"F243}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FA\symbol{"F244}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FA\symbol{"F245}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FA\symbol{"F246}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FA\symbol{"F247}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FA\symbol{"F248}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FA\symbol{"F249}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FA\symbol{"F24A}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FA\symbol{"F24B}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FA\symbol{"F24C}}}
\expandafter\def\csname faicon@clone\endcsname{{\FA\symbol{"F24D}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FA\symbol{"F24E}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FA\symbol{"F250}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FA\symbol{"F251}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FA\symbol{"F252}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FA\symbol{"F253}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FA\symbol{"F254}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FA\symbol{"F255}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FA\symbol{"F256}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FA\symbol{"F257}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FA\symbol{"F258}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FA\symbol{"F259}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FA\symbol{"F25A}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FA\symbol{"F25B}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FA\symbol{"F25C}}}
\expandafter\def\csname faicon@registered\endcsname{{\FA\symbol{"F25D}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FA\symbol{"F25E}}}
\expandafter\def\csname faicon@gg\endcsname{{\FA\symbol{"F260}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FA\symbol{"F261}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FA\symbol{"F262}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FA\symbol{"F263}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FA\symbol{"F264}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FA\symbol{"F265}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FA\symbol{"F266}}}
\expandafter\def\csname faicon@safari\endcsname{{\FA\symbol{"F267}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FA\symbol{"F268}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FA\symbol{"F269}}}
\expandafter\def\csname faicon@opera\endcsname{{\FA\symbol{"F26A}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FA\symbol{"F26B}}}
\expandafter\def\csname faicon@television\endcsname{{\FA\symbol{"F26C}}}
\expandafter\def\csname faicon@contao\endcsname{{\FA\symbol{"F26D}}}
\expandafter\def\csname faicon@500px\endcsname{{\FA\symbol{"F26E}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FA\symbol{"F270}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FA\symbol{"F271}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FA\symbol{"F272}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FA\symbol{"F273}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FA\symbol{"F274}}}
\expandafter\def\csname faicon@industry\endcsname{{\FA\symbol{"F275}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FA\symbol{"F276}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FA\symbol{"F277}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FA\symbol{"F278}}}
\expandafter\def\csname faicon@map\endcsname{{\FA\symbol{"F279}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FA\symbol{"F27A}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FA\symbol{"F27B}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FA\symbol{"F27C}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FA\symbol{"F27D}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FA\symbol{"F27E}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FA\symbol{"F280}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FA\symbol{"F281}}}
\expandafter\def\csname faicon@edge\endcsname{{\FA\symbol{"F282}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FA\symbol{"F283}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FA\symbol{"F284}}}
\expandafter\def\csname faicon@modx\endcsname{{\FA\symbol{"F285}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FA\symbol{"F286}}}
\expandafter\def\csname faicon@usb\endcsname{{\FA\symbol{"F287}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FA\symbol{"F288}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FA\symbol{"F289}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FA\symbol{"F28A}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FA\symbol{"F28B}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FA\symbol{"F28C}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FA\symbol{"F28D}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FA\symbol{"F28E}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FA\symbol{"F290}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FA\symbol{"F291}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FA\symbol{"F292}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FA\symbol{"F293}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FA\symbol{"F294}}}
\expandafter\def\csname faicon@percent\endcsname{{\FA\symbol{"F295}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FA\symbol{"F296}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FA\symbol{"F297}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FA\symbol{"F298}}}
\expandafter\def\csname faicon@envira\endcsname{{\FA\symbol{"F299}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FA\symbol{"F29A}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FA\symbol{"F29B}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FA\symbol{"F29C}}}
\expandafter\def\csname faicon@blind\endcsname{{\FA\symbol{"F29D}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FA\symbol{"F29E}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FA\symbol{"F2A0}}}
\expandafter\def\csname faicon@braille\endcsname{{\FA\symbol{"F2A1}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FA\symbol{"F2A2}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FA\symbol{"F2A3}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FA\symbol{"F2A4}}}
\expandafter\def\csname faicon@glide\endcsname{{\FA\symbol{"F2A5}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FA\symbol{"F2A6}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FA\symbol{"F2A7}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FA\symbol{"F2A8}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FA\symbol{"F2A9}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FA\symbol{"F2AA}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FA\symbol{"F2AB}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FA\symbol{"F2AC}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FA\symbol{"F2AD}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FA\symbol{"F2AE}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FA\symbol{"F2B0}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FA\symbol{"F2B1}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FA\symbol{"F2B2}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FA\symbol{"F2B3}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FA\symbol{"F2B4}}}


==> related.tex <==

Both clone detection and bug detection have been extensively studied in the literature for both traditional software programs and Ethereum smart contracts. Clone detection techniques utilize expensive symbolic transaction sketch~\cite{Eclone2018} or pair-wise signature comparison~\cite{He2019}. They can be applied to compiled contract bytecode, but efficiency is limited for checking contract-level similarities, instead of more fine-grained levels of granularity. More bug detection techniques have been developed for smart contracts (e.g., \cite{Bhargavan2016, brownformal, luu2016making, tsankov2018securify, tikhomirov2018smartcheck, delmolino2016step, Mueller2018}), while they often require manual efforts in defining specifications and/or bug patterns needed for validation and/or bug checking.

Machine learning and deep learning techniques have been used for clone detection (e.g., \cite{astnn2019,cclearner2017,White2016DeepLC}) and bug detection problems (e.g. \cite{Yang2015,Li2017}) in traditional software programs too, but little has been applied for smart contracts.

{\sc SmartEmbed} is unique in that it utilizes deep learning and similarity checking techniques to unify clone detection and bug detection together efficiently and accurately for Ethereum smart contracts. 

